HDArray: Parallel Array Interface for Distributed Heterogeneous Devices

Heterogeneous clusters with nodes containing one or more accelerators, such as GPUs, have become common. While MPI provides inter-address space communication, and OpenCL provides a process with access to heterogeneous computational resources, programmers are forced to write hybrid programs that manage the interaction of both of these systems. This paper describes an array programming interface that provides users with automatic and manual distributions of data and work. Using work distribution and kernel def and use information, communication among processes and devices in a process is performed automatically. By providing a unified programming model to the user, program development is simplified.

==> arxiv_hdarray/command.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%%  commands for names  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      
\newcommand{\name}{HDArray}
\newcommand{\mpi}{OpenMPI}
\newcommand{\region}{region}
\newcommand{\gdefsend}{{sGDEF}}
\newcommand{\gdefrecv}{{rGDEF}}
\newcommand{\gdefsendin}{{\gdefsend IN}}
\newcommand{\gdefsendout}{{\gdefsend OUT}}
\newcommand{\gdefrecvin}{{\gdefrecv IN}}
\newcommand{\gdefrecvout}{{\gdefrecv OUT}}
\newcommand{\sendmessage}{{SENDMSG}}
\newcommand{\receivemessage}{{RECVMSG}}
	
%%% interface prototype %%%  
\newcommand{\funcinit}{{\tt \name Init}}
\newcommand{\funccreate}{{\tt \name Create}}
\newcommand{\funcapplykernel}{{\tt \name ApplyKernel}}
\newcommand{\funcexit}{{\tt \name Exit}}
\newcommand{\funcread}{{\tt \name Read}}
\newcommand{\funcwrite}{{\tt \name Write}}
\newcommand{\funcreduce}{{\tt \name Reduce}}
\newcommand{\funcshow}{{\tt \name ShowDeviceInfo}}
\newcommand{\funcpartition}{{\tt \name Partition}}
\newcommand{\partitiontype}{{\tt PART\_T}}
\newcommand{\funcpatition}{{\tt \name UpdatePartition}}
\newcommand{\reduceop}{sum, product, max, and min}
\newcommand{\funcabsuse}{{\tt \name SetAbsoluteUse}}
\newcommand{\funcabsdef}{{\tt \name SetAbsoluteDef}}
\newcommand{\functrapezoiduse}{{\tt \name SetTrapezoidUse}}
\newcommand{\functrapezoiddef}{{\tt \name SetTrapezoidDef}}
\newcommand{\funcRegisterManUse}{{\tt \name RegisterUpdateUse}}
\newcommand{\funcRegisterManDef}{{\tt \name RegisterUpdateDef}}
\newcommand{\funcPtrUse}{{\tt updateUse}}
\newcommand{\funcPtrDef}{{\tt updateDef}}
\newcommand{\funcGetBoundaries}{{\tt \name GetBoundaries}}
\newcommand{\funcproto}[1]{{\tt #1}}

%\newcommand{\Samcomment}[1]{{\bf [#1]}}
%\newcommand{\Hyundokcomment}[1]{{\bf \color{Brown} [#1]}}
%\newcommand{\Okwancomment}[1]{{\color{Blue} [#1]}}
\newcommand{\Samcomment}[1]{}
\newcommand{\Hyundokcomment}[1]{}
\newcommand{\Okwancomment}[1]{}

%\newcommand{\pragma}{\#pragma parray \[clauses\]}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%% user defined packages  %%%%%%%%%%%%%%%%%  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
\usepackage{cite}

\usepackage[pdftex]{graphicx}
% declare the path(s) where your graphic files are
\graphicspath{{fig}}
% and their extensions so you won't have to specify these with
% every instance of \includegraphics
\DeclareGraphicsExtensions{.pdf,.jpeg,.png}

\usepackage[cmex10]{amsmath}
\interdisplaylinepenalty=2500

\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\algrenewcommand\textproc{}% Used to be \textsc

\usepackage{array}

\usepackage[caption=false,font=footnotesize]{subfig}

\usepackage{url}

\hyphenation{op-tical net-works semi-conduc-tor}

%\usepackage{outlines}
%%\usepackage{microtype}

\usepackage[english]{babel}
\usepackage{underscore}

\usepackage{tabularx}

\usepackage{listings}
\usepackage{color}
\usepackage[dvipsnames]{xcolor}
%\usepackage{sectsty}

\lstset{ 
%	language=C, % choose the language of the code
%	basicstyle=\fontfamily{pcr}\selectfont\footnotesize\color{red},
%	keywordstyle=\color{black}\bfseries, % style for keywords
%	numbers=none, % where to put the line-numbers
%	numberstyle=\tiny, % the size of the fonts that are used for the line-numbers     
%%	backgroundcolor=\color{darkgray},
%	showspaces=false, % show spaces adding particular underscores
%	showstringspaces=false, % underline spaces within strings
%	showtabs=false, % show tabs within strings adding particular underscores
%	frame=single, % adds a frame around the code
%	tabsize=2, % sets default tabsize to 2 spaces
%	rulesepcolor=\color{gray},
%	rulecolor=\color{black},
%	captionpos=b, % sets the caption-position to bottom
%	breaklines=true, % sets automatic line breaking
%	breakatwhitespace=false, 
	basicstyle=\tt\notsotiny,
	morekeywords={HDArrayInit, HDArrayExit,HDArrayApplyKernel,HDArrayWrite,HDArrayRead,HDArrayCreate,HDArrayPartition,use,def,pragma,hdarray, partition}
}

%\lstdefinestyle{base}{
%	language=C,
%	emptylines=1,
%	breaklines=true,
%	basicstyle=\notsotiny,
%	moredelim=**[is][{\color{red}]{@}{@},
%}

\newcommand*{\textsmallunderscore}{%
	\begingroup
	\fontencoding{T1}\fontfamily{lmtt}\selectfont
	\textunderscore
	\endgroup
}

\usepackage{microtype}
\usepackage[T1]{fontenc}
\usepackage[scaled]{beramono}
\newcommand\Small{\fontsize{7}{7}\selectfont}
\newcommand*\LSTfont{\Small\ttfamily\SetTracking{encoding=*}{-60}\lsstyle}

\newcommand{\BIBdecl}{\setlength{\itemsep}{0.3 em}}

\usepackage{verbatim}

\usepackage{enumitem}

\usepackage[export]{adjustbox}

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    
%%%%%%%%%%%%%%%%% user defined commands  %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    

%\makeatletter
%\renewcommand{\ALG@beginalgorithmic}{\footnotesize}
%\makeatother
%
%\algrenewcommand\alglinenumber[1]{\tiny #1:}
%
%\lstset{
%	basicstyle=\fontsize{7}{7.3}\selectfont\ttfamily
%}

\newcommand{\clearauthorinfo}{\author{No Author Given}
	\authorrunning{No Author Given}
	\institute{No Institute Given}}

\makeatletter
\newcommand\notsotiny{\@setfontsize\notsotiny\@vipt\@viipt}
\makeatother

\makeatletter
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
	{-8\p@ \@plus -4\p@ \@minus -4\p@}% make it 8
%	{-12\p@ \@plus -4\p@ \@minus -4\p@}%
	{-0.5em \@plus -0.22em \@minus -0.1em}%
	{\normalfont\normalsize\itshape}}
\makeatother


==> arxiv_hdarray/conclusion.tex <==
% \Mycomment{From design.tex}
% Because the \name\ interface supports heterogeneous devices, there are some opportunities to make the system more flexible and efficient. Recall that the \name\ runtime system automatically selects available devices and performs automatic partitioning. In other words, the system uses a fixed policy when the program starts. Then interesting questions arise. What if users want to utilize more on one device than the other? What about using different partitioning method for different kernels? Doing these automatically is beyond the scope of this paper, but we instead support a manual partitioning interface so that the users can further write highly optimized code.

% \Hyundokcomment{List of future work: 1. localization to utilize device memory. 2. advanced automatic distribution mentioned above. 3. load balancing. 4. running and evaluating deep learning neural network.  5. Tiling to optimize based on specific architecture architecture }
% \Hyundokcomment{What 1 or 2 item would be good to mention as future work?}

%\Hyundokcomment{List of future work: 1. localization to utilize device memory. 2. load balancing. }
We have presented the \name\ interface and runtime system for accelerator clusters. The interface features a novel global programming model which separates work partitioning from the concept of data distribution, thus enabling straightforward and flexible work distribution.

The interface abstracts away many low-level details of multiple address space programming, yet supports a low-level array programming environment through the \name\ annotations and APIs for performance tuning. We showed how the \name\ interface could help programmers to write and tune array-based programs for distributed devices. The offsets provide an intuitive and simple way to describe the access patterns of kernels, and the patterns can be easily changed by simply adjusting partitions without the modification of kernel code.

The \name\ runtime system performs efficient and fully automatic communication by managing the array sections. We presented optimizations including the caching mechanism and communication and computation overlap, which reduce or hide much of the overheads of communication detection.

Future work being considered is the ability to adjust work partitions assigned to devices.  This capability would allow splitting up computations to fit them in small device memories, and adjusting the sizes of work assigned to heterogeneous devices to provide load balancing.

%To make our runtime system more efficient and reliable, additional modifications are necessary. Unlike CPUs, accelerators typically have small physical memories, and only few devices support virtual addressing. To utilize the device memory, we can use a host buffer as a backing store to split the partitioned region to work with smaller data. 

%Another potential work is automatic load balancing. For \emph{regular} and \emph{repetitive} programs, in which the communication pattern is the same in all iterations, the runtime can analyze the performance of devices at each iteration and dynamically adjust work and data distributions.

\if{0}
\subsection{Future Work}
\label{subs:design_discuss}
With additional enhancements, the \name\ can be more efficient and reliable with a wider range of array-based programs. We discuss these now.
%Along with improving the programming model for non-regular programs, we plan to extend the system to be more scalable and to utilize device memory. 
%To make our programming model more efficient and reliable with general array-based programs, additional modifications may be necessary. We discuss our potentials and opportunities for the \name\ interface.

%\subsubsection{The Expressiveness of the Offset Clause}
%The offset helps users to write kernel code without considering communication; however, it cannot express non-regular, e.g., triangular, array access patterns of kernels. As a result, the users can only make conservative offsets for those kernels, causing unnecessary communication. 
%Instead of using ``relativeness'' of the offset, we can have users directly specify LUSE and LDEF for each device, similar to manual partitioning. To enhance the programming model, we can provide additional directive clauses and APIs for an easier way of expressing the absolute array sections for non-regular applications.

%While the offset helps users to write kernel code without considering communication, the offset cannot accurately express the fixed coordinates of array elements to be accessed because the offset is based on ``relativeness'' to the thread.  As a result, the users need to specify conservative offsets for kernels with non-regular, e.g., triangular, access pattern, causing unnecessary communication. 
%%As the system uses the offset information relative to each work item index for generating LDEF and LUSE, there is no good way to specify the offset for non-regular programs. 
%This can be solved by letting user directly specify LUSE and LDEF. To facilitate the programming model, we can provide additional directive clauses and APIs for easier way of expressing absolute array sections for non-regular applications.

\subsubsection{Handling Applications that Exceed Device Memory}
Unlike CPUs, accelerators typically have small physical memories and no virtual addressing.
The \name\ program will fail if the available device memory size is smaller than needed for computation because it allocates the entire array when \name s are created and uses the entire partitioned work item region for a kernel. To fit in the device memory, we can allocate the device buffer during the kernel computation and use a host buffer as a backing store to split the partitioned region to work with smaller data. This optimization is feasible by enhancing \funcapplykernel.

\subsubsection{Automatic Utilizations of Computational Resources}
The \name\ runtime does not support automatic load balancing. 
For \emph{repetitive} programs, in which the communication pattern is the same in all iterations of the serial loop enclosing kernel calls, the runtime can balance the work by analyzing the performance of devices at each iteration and dynamically adjust work and data distributions. Another utilization such as overlapping computation and communication is not also supported because of the SPMD execution model we use. The design of providing the overlap is ongoing future work.

%The \name\ system is flexible enough to compute on large data which cannot fit in the device memory by having a host memory as a backing store.
\fi

==> arxiv_hdarray/contribution.tex <==
%
% paper title
% can use linebreaks \\ within to get better formatting as desired


%	%
%	\title{Contribution Title\thanks{Supported by organization x.}}
%	%
%	%\titlerunning{Abbreviated paper title}
%	% If the paper title is too long for the running head, you can set
%	% an abbreviated paper title here
%	%
\title{ \name: Parallel Array Interface for Distributed Heterogeneous Devices}
\titlerunning{\name: Parallel Array Interface for Distributed Heterogeneous Devices}

%\author{Hyun Dok Cho\inst{1}\orcidID{0000-1111-2222-3333} \and
%	Okwan Kwon\inst{2}\orcidID{1111-2222-3333-4444} \and
%	Samuel P. Midkiff\inst{1}\orcidID{2222--3333-4444-5555}}
\author{Hyun Dok Cho\inst{1}\protect\footnote{This work was done while at Purdue University.} \and
	Okwan Kwon\inst{1} \and
	Samuel P. Midkiff\inst{2}}

%
\authorrunning{H. Cho et al.}
% First names are abbreviated in the running head.
% If there are more than two authors, 'et al.' is used.
%

\institute{
	NVIDIA Corporation, Santa Clara, CA 95050, USA\\
	\email{\{hyundokc,okwank\}@nvidia.com}
	\and
	Purdue University, West Lafayette, IN 47907, USA\\
	\email{smidkiff@purdue.edu} 
}

%\clearauthorinfo

%	%
\maketitle              % typeset the header of the contribution

==> arxiv_hdarray/design.tex <==
%
\begin{figure}[htb]
	\centering 
%	\vspace{-15pt}
	\subfloat[ The \name\ frontend]{\label{sf:sysA}  \includegraphics[width=0.47\textwidth]{fig/sysA2}}%
	\vspace{-2pt}
	\hskip 0.1truein
	\subfloat[ The \name\ runtime]{\label{sf:sysB}\includegraphics[width=0.46\textwidth]{fig/sysB4}}
%	\vspace{-5pt}
	\caption{An overview of the \name\ system within a single process.}
	\label{fig:overview}
	\vspace{-10pt}
\end{figure}
%
We now present the design of the \name\ interface and its runtime system as shown in Fig.~\ref{fig:overview}.
%, which provides an efficient and straightforward array programming model. 
The central structure, and concept, of the \name\ system is the \name\ itself.  
%An \name\ consists of a {\em host buffer}; a {\em device buffer}; sets of global definitions ({\em GDEF set}); a set of local definitions ({\em LDEF set}); a set of local uses ({\em LUSE set}); history information used to minimize runtime overheads; and process information.
The \name\ encapsulates a {\em host buffer} and {\em device buffer} by keeping necessary states for communication among processes and kernel computation.
%
%In addition to these data structures, which are transparent to the programmer, the \name\ system provides a collection of APIs and annotations that the 
The \name\ system provides a collection of APIs and annotations that the programmer uses to access the features of the \name\ system.  These APIs and annotations are translated by the \name\ frontend into calls, arguments, and initialization files (M) for use by the \name\ runtime.

\subsection{\name\ Structures}
\label{subs:structures}

Each MPI process that maps to a single OpenCL device maintains \name s and their structures. Each \name\ contains the necessary state for the system to automatically generate communication and manage data distributions.
%Each process matches a single OpenCL context and device, and maintains these structures for each \name. 

%\paragraph{Host and device buffers} contain the distributed data for an \name\ for a host and device in the \name\ program, respectively. Host buffers reside in the process memory of the host, and device buffers reside on a device. 
%
%\paragraph{The \textbf{\textit{LDEF}} and \textbf{\textit{LUSE}} sets.} Each process maintains LDEF and LUSE sets for each \name , where each set describes local definition and use sets for each process.  
%The local definition and use information is summarized as a range of $ [{\it Lower bound}, {\it Upper bound}] $, and LDEF and LUSE are a set of these ranges.
%
%\paragraph{The \textbf{\textit{GDEF}} sets: \gdefsend\ and \gdefrecv.}  
%Like LDEF and LUSE, these are sets of sets,  containing global definition information for every \name\ and maintained by every process. \gdefsend\ for a process $ p $ describes \name\ elements that $ p $ has written, but not sent, to other processes $ q $, i.e., the elements for which $ p $ describes the coherent copy that must be sent to other processes that use those values. \gdefrecv\ for process $ p $ describes elements of the \name\ that $ p $ has not received from $ q $.

Host and device buffers contain the distributed data for an \name\ for a host and device in the \name\ program, respectively. Host buffers reside in the process memory of the host, and device buffers reside on a device. 

An \name\ contains sets of array sections: {\em global}, i.e., across all kernels, definition sections ({\em GDEF}); {\em local}, i.e., for a particular kernel, definition sections ({\em LDEF}); and local use sections ({\em LUSE}). 
These sets are summarized by one or more sections of [LB:UB] that give the lower and upper bounds of the array sections for all processes. 
%To be more precise, 
GDEF is a set of written sections not propagated to different processes, and %each process maintains GDEF sets for all processes.  
two types of GDEFs are maintained: \gdefsend\ and \gdefrecv. 
\gdefsend\ for a process $ p $ describes \name\ elements that $ p $ has written, but not sent, to other processes $ q $,
i.e., the elements for which $ p $ describes the coherent copy that must be sent to other processes that use those values.
\gdefrecv\ for process $ p $ describes elements of the \name\ that $ p $ has not received from $ q $.
LUSE/LDEF is the set of sections each process reads/writes in the kernel.

\name\ programs are SPMD programs, and each process maintains coherent local copies of the aforementioned four sets for all processes,  
%and each process knows the number of processes, its rank, and the \name\ calls made by other processes. 
and thus each process knows the array access information of the other processes.
%
%Each process maintains coherent local copies of the four sets for all processes without communicating with other processes. 
%This is possible because \name\ programs are SPMD programs, 
%%and each process knows the number of processes, its rank, and the \name\ calls made by other processes. 
%and thus each process knows the array access information of the other processes.
%
All LUSE, LDEF, and GDEF sets are empty when an \name\ is created. LUSE (LDEF) is updated by \name\ annotations and APIs, as discussed in Section~\ref{subs:ui}, and GDEF is updated as a function of itself, LUSE, and LDEF, which we describe in Section~\ref{subs:comm_gen}. 
%With these sets, the runtime communicates elements of \name s immediately before a kernel launch.
%
%LDEF and LUSE sets for each \name , where each set describes local definition and use sets for each process.  
%The local definition and use information is summarized as a range of $ [{\it Lower bound}, {\it Upper bound}] $, and LDEF and LUSE are a set of these ranges.

As well, each process maintains a history of  local and global sections, and sections to communicate for each \name\ of a kernel. The runtime maintains the history to reduce the overhead of determining communication by avoiding an expensive data flow evaluation if possible, as described in Section~\ref{subs:optimization}.

\subsection{Communication Generation using GDEF, LDEF, and LUSE}
\label{subs:comm_gen}
%\paragraph{{\textit{Communication Generation}}.}  
The runtime communicates elements of \name s immediately before a kernel launch. Intersecting the GDEF and LUSE sets allows a process to determine which processes have elements of an \name\ that it will use in a kernel call, and therefore which elements it must communicate with that process.  
%By intersecting its GDEF information with the LUSE information maintained for each process, a process can determine which processes it must send array elements.
%After the communication and execution of some kernel $ k $, GDEF sets for each \name\ $ h $ used in the kernel must be updated to reflect the changes in the data received or defined because of the kernel invocation. This is done by Eqn.~\ref{eq:subtract_send}. and~\ref{eq:subtract_recv}, where each process $ p $ computes for all other processes $ j, j /neq j $: \Hyundokcomment{Should I reflect the changes ($ {\gdefsendout}_{H_k,i}(j) $) to Fig. 2. as well?}\Samcomment{Yes, once we all agree this is correct.}
%%{\small
%\begin{align}
%{\gdefsendout}_{h,p}(j) = {\gdefsendin}_{h,p}(j) - {\gdefsendin}_{h,p}(j) \cap {\it LUSE}_{h,p}(j)\label{eq:subtract_send}\\
%{\gdefrecvout}_{h,p}(j) = {\gdefrecvin}_{h,p}(j) - {\gdefrecvin}_{h,i}(j) \cap {\it LUSE}_{h,p}(p)\label{eq:subtract_recv}
%\end{align}
%Note that Eqn.~\ref{eq:subtract_send} and~\ref{eq:subtract_recv} differ in which {\it LUSE} of processes to intersect.
%%}%
%%
%%\begin{equation}
%%{\it GDEFOUT}(k) = {\it GDEFIN}(k) - {\it GDEFIN}(k) \cap {\it LUSE}(k)\label{eq:subtract}
%%\end{equation}
%These updates remove from the GDEF of every process $ i $, the sections process $ i $ sent to (or received from) process $ j $  to prevent them from being sent (or received) again at the next communication, unless the section is redefined. Fig.~\ref{fig:designcomm} shows how the system maintains the GDEF with two processes.
%Similarly, for all \name\ $ H_k $ that is {\em defined} in kernel call $ k $ and for all other processes $ j \neq i$, each process $ i $ computes:
%%{\small
%\begin{align}
%{\gdefsendout}_{h,p}(j) = {\gdefsendin}_{h,p}(j) \cup {\it LDEF}_{h,p}(p) \label{eq:union_send}\\
%{\gdefrecvout}_{h,p}(j) = {\gdefrecvin}_{h,p}(j) \cup {\it LDEF}_{h,p}(j) \label{eq:union_recv}
%\end{align}
%%}%
%%
%%\begin{equation}
%%{\it GDEFOUT}(k) = {\it GDEFIN}(k) \cup {\it LDEF}(k) \label{eq:union}
%%\end{equation}
%which unions the LDEF into its GDEF, since the process now contains the coherent copy of these newly defined array elements and may need to communicate them at future kernel calls.
%
\begin{figure*}[htb]
	\centering
	%	\vspace{-5pt}
	\subfloat{\includegraphics[max width=4.6in]{fig/designcomm4}}%
	%	\subfloat{\includegraphics[width=4.5in]{fig/designcomm3}}%
	\vspace{-10pt}
	\caption{\gdefsend\ of \emph{use} \name\ for Process 0 before and after kernel call (\gdefsend$_{0,1}$($ l $) and \gdefsend$_{0,1}$($ k $) respectively). The system intersects \gdefsend\ with LUSE, sends the intersection from P\textsubscript{0} to P\textsubscript{1}, and updates \gdefsend. Note that LDEF$_{0,0}$($ k $) is NULL.}
	\label{fig:designcomm}
	\vspace{-13pt}
\end{figure*}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%After the communication, GDEF sets for each \name\ \emph{used} in the kernel must be updated to avoid redundant communication, as shown in  Eqn.~\ref{eq:subtract_send} and~\ref{eq:subtract_recv}. 
%Let $ k $ be the index of a kernel call and $ l $ the set of all preceding kernel calls of $ k $.  
%For process $ p $, \gdefsendin$_{p}$(k)  and \gdefrecvin$_{p}$(k) are sets of sections that are live before the kernel call $ k $, which can be calculated as follows:
%\Hyundokcomment{Should I reflect the changes ($ {\gdefsendout}_{H_k,i}(j) $) to Fig. 2. as well?}\Samcomment{Yes, once we all agree this is correct.}
%{\small
%\begin{align}
%{\gdefsendin}_{p}(k) = {\gdefsendout}_{p}(l) - {\it LUSE}(k)\label{eq:subtract_send}\\
%{\gdefrecvin}_{p}(k) = {\gdefrecvout}_{p}(l) - {\it LUSE}_{p}(k)\label{eq:subtract_recv}
%\end{align}
%Note that Eqn.~\ref{eq:subtract_send} and~\ref{eq:subtract_recv} differ in which LUSE of processes to intersect. LUSE$_{p}$(k) is local uses by process $ p $ for the kernel call $ k $, whereas LUSE(k) represents all  LUSE$_{q}$(k) for $ 0 \leq q \leq nprocs - 1, q \neq p $.
%}%
%These updates remove from the GDEF of every process $ p $, the sections process $ p $ sent to (or received from) process $ q $  to prevent them from being sent (or received) again at the next communication, unless the section is redefined. Fig.~\ref{fig:designcomm} shows how the system maintains the \gdefsend\ with two processes.
%
%Similarly, after the kernel execution, the system updates \gdefsendout$_{p}$(k) and \gdefrecvout$_{p}$(k) which are sets of sections that are live after the kernel call $ k $. 
%For all \name\ that is {\em defined} in kernel call $ k $, each process $ p $ computes:
%{\small
%\begin{align}
%{\gdefsendout}_{p}(k) = {\gdefsendin}_{p}(k) \cup {\it LDEF}_{p}(k) \label{eq:union_send}\\
%{\gdefrecvout}_{p}(k) = {\gdefrecvin}_{p}(k) \cup {\it LDEF}(k) \label{eq:union_recv}
%\end{align}
%}%
%which unions the LDEF into its GDEF, since the process now contains the coherent copy of these newly defined array elements and may need to communicate them at future kernel calls.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Fig.~\ref{fig:designcomm} shows the example of the intersection with two processes.
Let $ k $ be the index of a kernel call and $ l $ the preceding kernel call of $ k $.
For process $ p $, \gdefsend$_{p,q}$($ l $)  and \gdefrecv$_{p,q}$($ l $) are sets of sections that are live before the kernel call $ k $. 
LUSE$_{p,p}$($ k $) is local uses by process $ p $ for the kernel call $ k $, whereas LUSE$_{p,q}$($ k $) represents  local uses of other process $ q $ for $ 0 \leq q \leq nprocs - 1, q \neq p $. 
The communication messages of $ p $ to send and receive for the kernel call $ k $ are then generated as:
{\small
\begin{align}
{\it \sendmessage}_{p,q}(k) = {\it \gdefsend}_{p,q}(l)  \cap {\it LUSE}_{p,q}(k) \label{eq:intersectionsend}\\
{\it \receivemessage}_{p,q}(k) = {\it \gdefrecv}_{p,q}(l)  \cap {\it LUSE}_{p,p}(k) \label{eq:intersectionrecv}
\end{align}
}%
%
After communication and kernel execution, GDEF sets for each \name\ for kernel call $ k $ must be updated to avoid redundant communication for used \name s, and detect new communication in the future kernel call $ k + 1 $ for defined \name s. These updates can be calculated together as Eqns.~\ref{eq:update_gdef_send} and~\ref{eq:update_gdef_recv}. 
%
{\small
\begin{align}
{\gdefsend}_{p,q}(k) = ({\gdefsend}_{p,q}(l) - {\sendmessage}_{p,q}(k)) \cup {\it LDEF}_{p,p}(k) \label{eq:update_gdef_send}\\
{\gdefrecv}_{p,q}(k) = ({\gdefrecv}_{p,q}(l) - {\receivemessage}_{p,q}(k)) \cup {\it LDEF}_{p,q}(k) \label{eq:update_gdef_recv}
\end{align}
}%
%
Fig.~\ref{fig:designcomm} shows the example of the \gdefsend\ update. 
The \sendmessage\ and \receivemessage\ for the kernel call $ k $ are subtracted from \gdefsend\ and  \gdefrecv\ of kernel call $ l $, respectively. These removes communicated data from \gdefsend\ and \gdefrecv\ of the kernel call $ l $. The results of the subtractions are then unioned with LDEF sets to update \gdefsend\ and \gdefrecv\ for kernel call $ k $. 
Similar to LUSE, LDEF$_{p,p}$($ k $) and LDEF$_{p,q}$($ k $) sets represent local definitions by process $ p $ and $ q $ for kernel call $ k $, respectively. 

%\paragraph{Process and history information}  
%Each process maintains information about its rank, the  number of processes, and the distribution of the \name s.  As well, each process maintains, for each \name, a history of prior local and global sections, and intersections to reduce the overhead of determining communication by avoiding an expensive data flow evaluation if possible, as described in Section~\ref{subs:optimization}.

\section{\name\ Programming Interface}
%\subsection{\name\ Programming Interface}
\label{subs:ui}
The \name\ programming interface has two types of specifications. First, a single pragma of the form {\tt \#pragma hdarray [clauses]} allows user-defined hints for generating LUSE and LDEF to find data to be accessed, and partitioning work item regions to distribute work.  The functionality is contained in the clauses, described next.  Second, \name\ provides library functions, hiding low-level details of distributed device programming, described below.
Hereafter, we use the terms work item and thread interchangeably. 

%\subsection{\name\ Pragmas}  
%\name~ provides annotations, with a {\tt \#pragma \MakeLowercase{\name}} statement with clauses.

%The pragmas allow the specification of data read and written for communication handling and manually partitioning for communication tuning.
%
%\subsubsection{Pragma Clauses}
\label{subs:clauses}
%
Table~\ref{tab:clauses} lists the available annotation clauses. Five clauses exist: {\em use}, {\em def}, {\em use@}, {\em def@},  and {\em partition}.  We now explain each of these.

\begin{table}[tb]
	\notsotiny
	\renewcommand{\arraystretch}{1.3}
%		\vspace{-10pt}
	\caption{Core \MakeLowercase{\name} directive clauses}
	\begin{center}
		\vspace{-13pt}
		\resizebox{\columnwidth}{!}{%
			\begin{tabular}{|l|l|}
				\hline
				\bf Clause & \bf Description\\
				\hline
				\emph{use} (array name, offset) & Declare offset(s) of an array to be used.\\
				\hline
				\emph{def} (array name, offset) & Declare offset(s) of an array to be defined.\\
				\hline
				\emph{use@} (array name) & Declare absolute sections(s) of an array to be used.\\
				\hline
				\emph{def@} (array name) & Declare absolute sections(s) of an array to be defined.\\
				\hline
				\emph{partition} (partition ID, dimension, dev:ID, region) & Manually partition work item regions to devices.\\
				\hline
			\end{tabular}
		}
%		\vspace{-25pt}
		\vspace{-10pt}
	\end{center}
	\label{tab:clauses}
\end{table}
%
%\begin{table}[t]
%\notsotiny%
%	\renewcommand{\arraystretch}{1.15}
%%	\vspace{-3pt}
%	\caption{Example specifications of offsets for \emph{use} and \emph{def} clauses}
%	\begin{center}	
%		\vspace{-5pt}
%%		\resizebox{\columnwidth}{!}{%
%			\begin{tabular}{|l|l|l|}
%				\hline
%				\bf Dimension & \bf Offset & \bf Description.\\
% 				\hline
%				1D & (-1) & Access previous element in dimension 1 (dim1). \\
%				\hline
%				2D & (0, +1) & Access next element of the row (dim1).\\
%				\hline
%				3D & (0, 0, *) &  Access all elements in dim3.\\
%				\hline
%			\end{tabular}
%%		}
%		\vspace{-20pt}
%	\end{center}
%	\label{tab:offsets}
%\end{table}

\paragraph{Offset Clauses: \textbf{\textit{use}} and \textbf{\textit{def}}.} 
Each \name\ accessed in a kernel can be a \emph{use}, \emph{def}, or both. These clauses specify elements of arrays, as offsets relative to work items, that will be read and/or written by a single work item. The offsets can be used when a kernel's array access pattern is relative to a work item, which is the most common kernel programming pattern. If the offsets are specified, the system derives LDEF and LUSE from the offset and partitioned work item region for each process. 
An offset can be any integer, e.g., ``0'' indicates the current position of an array element relative to the work item index. It also describes a direction with $``+"$ or $``-"$; e.g., $(0, -1)$, referring to the previous elements of the same row. An $``*"$ denotes all elements of the array in the dimension of interest, e.g., $(0, *)$ denotes all elements in a row of a 2-dimensional array.%, and is the offset of array A in Listing~\ref{code:device}. 

\paragraph{Absolute Section Interface Clauses: \textbf{\textit{use@}} and \textbf{\textit{def@}}.}
\label{subs:absclause} 
When it is difficult to represent offsets, e.g., a kernel's access pattern is not relative to a work item or non-rectangular, one can use the \emph{absolute section interface} with \emph{use@} and/or \emph{def@} clauses and APIs.
%When different work items on devices have different access patterns, or a non-rectangular pattern is accessed, the \emph{use} and \emph{def} offsets above are insufficient.  For these cases, \name\ provides an \emph{absolute section interface} using \emph{use@} and \emph{def@} clauses, and APIs.  
Unlike offsets, absolute sections are the coordinates of the [lowerbound, upperbound] of each dimension of an up to three dimensional item.  The absolute section interface clauses inform the system to bypass LUSE/LDEF updates (Fig.~\ref{fig:applykernel}).  Instead, users call absolute section interface APIs, e.g., \funcabsuse, described in Section~\ref{ssub:api}, to set LDEF and LUSE.  The APIs allow users to specify multiple absolute sections for each device, allowing non-rectangular regions or different access patterns for each device to be described, and enable fine tuning of communication. %]\Samcomment{How?  This seems to describe rectangular}.  \Hyundokcomment{Updated the paragraph. The \emph{use@} and \emph{def@} clauses simply tell the system to bypass the local section updates. Actually, the absolute section can be described using APIs (\funcabsuse, \funcabsdef, and \functrapezoid). The first two functions can be called multiple times so that non-rectangular shape can be described in line-by-line fashion. The last function can describe both trapezoidal and triangular shape. Should we create another sub-section, say "Absolute Section Interface", that discuss both clauses and APIs together? Right now, these are spread to two different sub-sub-sections, "Pragma Clauses" and "\name~Library Functions".}

\paragraph{Partition Clause: \textbf{\textit{partition}}.} 
\name\ provides an  \funcpartition\ library call that allows a ROW, COL or BLOCK partition to be specified.  \name\ will automatically partition the work evenly across processes and devices in the specified manner.  A ROW partitioning is shown in Listing~\ref{code:host}.  The API then returns  a unique partition ID, which is used, repeatedly if necessary, to execute kernels with the partitioned work item. This partition ID, along with {\it use} and {\it def} information, allows the system to know data needed by the work done by the kernel on each device. 
%. \Hyundokcomment{Changed the "annotation" to "API", and move annotation expansion to below. Here the API is \funcpartition. This paragraph is actually about pragma clause (annotation). Should I move the sentences above to somewhere else or does it look okay?}

%\name~provides both annotation and an API that partition a work item region for each processes to distribute both work and data. Once partitioning is done, the system generates an unique partition ID which can be used to create LDEF and LUSE, and execute kernel with the partitioned work item regions. Specifically, the \emph {partition} clause allows the manual\footnote{The partition API evenly partitions the regions as mentioned in Section~\ref{ssub:api}.} specification of the partition of the region onto devices. The \name~frontend then expands the annotation to an internal function call that performs the partitioning and makes a partition ID available.

\begin{lstlisting}[caption={Manually partitioned Correlation host code.},label={code:partition}, frame=lines, breaklines=true, xleftmargin=2em, framexleftmargin=1.5em, numbers=left, numberstyle=\tiny, numbersep=5pt, captionpos=b, float=tb, belowskip=-3.5em, aboveskip=-0em]
...
#pragma hdarray partition(part0,        (10240,10240),\
                          dev:0,   (0,3008),(0,10240),\  
                          dev:1,(3008,7232),(0,10240))
...
HDArrayApplyKernel("corr_ker1", part0, ... );
HDArrayApplyKernel("corr_ker2", part0, ... );
...
\end{lstlisting}

The \name\ pragma enables manual partitions to be used as well, as shown in Listing~\ref{code:partition}, which specifies two work regions.  The annotation is expanded to an internal function call that performs the partitioning and returns  a unique partition ID. In lines 6-7, the partition ID ({\tt part0}) is used to determine the work distributions of the two kernels.  This annotation allows more programmer control for optimal communication tuning and load balancing.

%Listing~\ref{code:partition} shows the manual definition of a partition specifying different layout of regions for two devices in the {\tt hdarray} pragma.  In the two following calls on lines 6-7, the paritition ID ({\tt part0}) is used to determine the work distributions of the two kernels. This is beneficial because different kernels may need different work distribution for load balancing of work across devices, or using a partial devices when this is more efficient than communicating the data. Although manual partitioning requires understanding of the communication patterns of the kernels, it gives more control and flexibility to programmers. 

%\subsubsection{\name\ Library Functions}
\subsection{\name\ Library Functions}
\label{ssub:api}
The library functions, with core APIs described in Table~\ref{tab:prototype}, encapsulate low-level details of the programming model.
%and are discussed in detail in Section~\ref{subs:executinphase}.

%\begin{table*}[!ht]
%\tiny
%	\renewcommand{\arraystretch}{1.2}
%	\centering
%	\caption{\name\ Core interface library functions}
%%	\vspace{-5pt}
%	\begin{tabularx}{\textwidth}{|X|X|}
%		\hline
%		 int \funcinit(int argc, char *argv[], char *kpath, char *dpath) & 
%		 Initialize \name\ runtime environment. Returns device ID.
%		 kpath is the path to the OpenCL kernel file and dpath (optional) is the path to the device information file.\\
%		\hline
%		void \funcexit(void) & 
%		Terminate the \name\ runtime environment.\\
%		\hline
%		void \funcshow(int deviceID) & 
%		Display a mapping from each MPI rank to devices and device information. Takes a deviceID which is the same as the MPI rank.\\
%		\hline	
%		\name\_t *\funccreate(char *symbol, char *type, void *buf, int dim, ... ) & 
%		 Allocate array to host and device buffer and returns a \name\ handle. 
%		 The 1st and 2nd parameters are the name and type of an array. Takes a variable argument list for the array size. \\
%		\hline
%		int \funcpartition(HDARRAY_PARTITION part, int dim, ... ) & 
%		Partition work item regions. The 1st parameter is type of partitioning. Takes a variable argument list for the array size and regions for each dimension. The list of currently supported partitions: ROW, COL, and BLOCK.\\
%		\hline
%		void \funcapplykernel(char *kernalName, int partitionID, ... ) & 
%		Perform communication and kernel execution. 
%		Takes the kernel name, partition ID, and kernel arguments. The order of the kernel arguments must be identical to the order of kernel parameters. \\
%		\hline
%		void \funcread(\name\_t *HDArr, void *userArr, int partitionID) & 
%		Read an array section from the \name\ object (HDArr) to host memory (userArr). 
%		Takes partition ID that specifies the array section to be read.\\
%		\hline
%		void \funcwrite(\name\_t *HDArr, void *userArr, int partitionID) & 
%		Write an array section to an \name\ object (HDArr) from host memory (userArr). 
%		Takes partition ID that specifies the array section to be written.\\
%		\hline
%		void \funcreduce(\name\_t *HDArr, void *res, HDARRAY\_REDUCE\_OP op, int partitionID) & 
%		Reduce specific array sections to a scalar value and copy it to res. \\ % The list of currently supported ops: HDARRAY_REDUCE_SUM, HDARRAY_REDUCE_PRODUCT, HDARRAY_REDUCE_MAX, and HDARRAY_REDUCE_MIN.
%		\hline
%		void \funcabsuse(char *kernalName, int partitionID, \name\_t *HDArr, int deviceID, int dim, ... ) & 
%		Set absolute section used (LUSE) for each device. \\
%		\hline
%		void \funcabsdef(char *kernalName, int partitionID, \name\_t *HDArr, int deviceID, int dim, ... ) & 
%		Set absolute section defined (LDEF) for each device.\\ 
%		\hline
%		void \functrapezoiduse(char *kernalName, int partitionID, \name\_t *HDArr, int deviceID, int dim, ... ) & 
%		Predefined shape for LUSE. Specify four positions of upper-left, upper-right, below-left, and below-right.\\ 
%		\hline
%		void \functrapezoiddef(char *kernalName, int partitionID, \name\_t *HDArr, int deviceID, int dim, ... ) & 
%		Predefined shape for LDEF. Specify four positions of upper-left, upper-right, below-left, and below-right.\\ 
%		\hline
%%		region_t **\funcGetBoundaries(int partID) & Get boundary information of a partition for all devices.\\
%%		\hline
%%		void (*\funcPtrUse)(char *kernalName, int partitionID, \name_t *arr) &  User function that updates LUSE.\\
%%		\hline
%%		void (*\funcPtrDef)(char *kernalName, int partitionID, \name_t *arr) &  User function that updates LDEF.\\
%%		\hline			
%%		void \funcRegisterManUse(char *kernalName, int partitionID, \name_t *arr, void (*\funcPtrUse)( ... ))&  Register user function to \funcPtrUse.\\
%%		\hline
%%		void \funcRegisterManDef(char *kernalName, int partitionID, \name_t *arr, void (*\funcPtrDef)( ... )) &  Register user function to \funcPtrDef.\\			
%%		\hline
%	\end{tabularx}
%	\label{tab:prototype}
%	\vspace{-10pt}
%\end{table*}

\begin{table*}[t]
	\notsotiny
	\renewcommand{\arraystretch}{1.2}
	\centering
%	\vspace{-10pt}
	\caption{Core \name\ interface library functions}
		\vspace{-8pt}
	\begin{tabularx}{\textwidth}{|X|X|}
		\hline
		\multicolumn{1}{|c|}{\textbf{Prototype}} & \multicolumn{1}{c|}{\textbf{Description}} \\
		\hline
		\funcproto{int \funcinit(int argc, char *argv[], char *kpath, char *dpath)} & 
		Initialize \name\ runtime environment and returns device ID.
		Take path to OpenCL kernel file ({\tt kpath}) and optional device information file ({\tt dpath}).\\
%		kpath is the path to the OpenCL kernel file and dpath (optional) is the path to the device information file.\\
		\hline
		\funcproto{void \funcexit(void)} & 
		Terminate the \name\ runtime environment.\\
		\hline
		\funcproto{void \funcshow(int devID)} & 
		Display device information. Take device ID.\\ %(MPI rank).\\
		\hline	
		\funcproto{\name\_t *\funccreate(char *sym, char *type, void *uA, int dim, ... )} & 
		Allocate host and device buffer and returns \name\ handle. 
		Take name, type, address, and size of user array ({\tt uA}).\\
%		The 1st and 2nd parameters are the name and type of an array. Takes a variable argument list for the array size. \\
		\hline
		\funcproto{int \funcpartition(\partitiontype\ type, int dim, ... )} & 
		Partition work item regions. Take type of partition and variable list for  array size and region for each dimension.  Supported types: {\tt ROW}, {\tt COL}, and {\tt BLOCK}.\\
		\hline
		\funcproto{void \funcapplykernel(char *kName, int partID,...)} & 
		Perform communication and kernel execution. 
		Take the kernel name, partition ID, and kernel arguments. \\
		\hline
		\funcproto{void \funcread(\name\_t *hA, void *uA,int partID)} \newline 
		$\Rightarrow$ Same for \funcwrite & 
		Read(Write) array section specified by partition ID from(to) \name({\tt hA}) to(from) user array ({\tt uA}).\\
		\hline
		\funcproto{void \funcreduce(\name\_t *hA, void *res, REDUCE\_OP op, int partID)} & 
		Reduce specific array sections of \name({\tt hA}) to a scalar value({\tt res}). Supported ops: {\tt SUM}, {\tt PROD}, {\tt MAX}, and {\tt MIN}.\\
		\hline
		\funcproto{void \funcabsuse(char *kName, int partID, \name\_t *hA, int devID, int dim, ... )} \newline 
		$\Rightarrow$ Same for \funcabsdef & 
		Set absolute section used(defined) for each device. The absolute section becomes LUSE(LDEF). \\
		\hline
		\funcproto{void \functrapezoiduse(char *kName, int partID, \name\_t *hA, int devID, int dim, ... )} \newline 
		$\Rightarrow$ Same for \functrapezoiddef & 
		Set predefined shape for LUSE(LDEF). Specify four positions of upper-left, upper-right, below-left, and below-right.\\ 
		\hline
		% \funcproto{void (*\funcPtrUse)(char *kName, int partID, \name_t *hA)} \newline
		% $\Rightarrow$ Same for \funcPtrDef & 
		% User function that updates LUSE(LDEF).\\
		% \hline
		% \funcproto{void \funcRegisterManUse(char *kName, int partID, \name_t *hA, void (*\funcPtrUse)( ... ))} \newline
		% $\Rightarrow$ Same for \funcRegisterManDef & 
		% Register user function to \funcPtrUse(\funcPtrDef).	\\
%		 \hline
%				region_t **\funcGetBoundaries(int partID) & Get boundary information of a partition for all devices.\\
%				\hline
%				void (*\funcPtrUse)(char *kernalName, int partitionID, \name_t *arr) &  User function that updates LUSE.\\
%				\hline
%				void (*\funcPtrDef)(char *kernalName, int partitionID, \name_t *arr) &  User function that updates LDEF.\\
%				\hline			
%				void \funcRegisterManUse(char *kernalName, int partitionID, \name_t *arr, void (*\funcPtrUse)( ... ))&  Register user function to \funcPtrUse.\\
%				\hline
%				void \funcRegisterManDef(char *kernalName, int partitionID, \name_t *arr, void (*\funcPtrDef)( ... )) &  Register user function to \funcPtrDef.\\			
%				\hline
	\end{tabularx}
	\label{tab:prototype}
	\vspace{-15pt}
\end{table*}

%\begin{table*}[ht]
%	\notsotiny
%	\renewcommand{\arraystretch}{1.2}
%	\centering
%	\vspace{-10pt}
%	\caption{\name\ interface library functions}
%	\vspace{-5pt}
%	\begin{tabularx}{\textwidth}{|X|}
%		\hline
%%		\multicolumn{1}{|c|}{\textbf{Prototype}} & \multicolumn{1}{c|}{\textbf{Description}} \\
%%		\hline
%		\funcproto{int \funcinit(int argc, char *argv[], char *kpath, char *dpath)} 
%		\newline
%		$\Rightarrow$Initialize \name\ runtime environment and returns device ID.
%		Take path to OpenCL kernel file (kpath) and optional device information file (dpath).\\
%		%		kpath is the path to the OpenCL kernel file and dpath (optional) is the path to the device information file.\\
%		\hline
%		\tt{void \funcexit(void)} 
%		\newline 
%		$\Rightarrow$Terminate the \name\ runtime environment.\\
%		\hline
%		\funcproto{void \funcshow(int devID)} 
%		\newline 
%		$\Rightarrow$Display device information. Take device ID.\\ %(MPI rank).\\
%		\hline	
%		\funcproto{\name\_t *\funccreate(char *sym, char *type, void *uA, int dim, ... )} 
%		\newline 
%		$\Rightarrow$Allocate host and device buffer and returns \name\ handle. 
%		Take name, type, address, and size of user array (uA).\\
%		%		The 1st and 2nd parameters are the name and type of an array. Takes a variable argument list for the array size. \\
%		\hline
%		\funcproto{int \funcpartition(\partitiontype\ type, int dim, ... )} 
%		\newline 
%		$\Rightarrow$Partition work item regions. Take type of partition and variable list for  array size and region for each dimension.  Supported types: ROW, COL, and BLOCK.\\
%		\hline
%		\funcproto{void \funcapplykernel(char *kName, int partID,...)} 
%		\newline 
%		$\Rightarrow$Perform communication and kernel execution. 
%		Take the kernel name, partition ID, and kernel arguments. \\
%		\hline
%		\funcproto{void \funcread(\name\_t *hA, void *uA,int partID)} \newline 
%		$\Rightarrow$Same prototype for \funcwrite 
%		\newline 
%		$\Rightarrow$Read(Write) array section specified by partition ID from(to) \name(hA) to(from) user array (uA).\\
%		\hline
%		\funcproto{void \funcreduce(\name\_t *hA, void *res, REDUCE\_OP op, int partID)} 
%		\newline 
%		$\Rightarrow$Reduce specific array sections of \name(hA) to a scalar value(res). Supported ops: SUM, PROD, MAX, and MIN.\\
%		\hline
%		\funcproto{void \funcabsuse(char *kName, int partID, \name\_t *hA, int devID, int dim, ... )} \newline 
%		$\Rightarrow$Same prototype for \funcabsdef 
%		\newline 
%		$\Rightarrow$Set absolute section used(defined) for each device. The absolute section becomes LUSE(LDEF). \\
%		\hline
%		\funcproto{void \functrapezoiduse(char *kName, int partID, \name\_t *hA, int devID, int dim, ... )} \newline 
%		$\Rightarrow$Same prototype  for \functrapezoiddef
%		\newline 
%		$\Rightarrow$Set predefined shape for LUSE(LDEF). Specify four positions of upper-left, upper-right, below-left, and below-right.\\ 
%		\hline
%		%		region_t **\funcGetBoundaries(int partID) & Get boundary information of a partition for all devices.\\
%		%		\hline
%		%		void (*\funcPtrUse)(char *kernalName, int partitionID, \name_t *arr) &  User function that updates LUSE.\\
%		%		\hline
%		%		void (*\funcPtrDef)(char *kernalName, int partitionID, \name_t *arr) &  User function that updates LDEF.\\
%		%		\hline			
%		%		void \funcRegisterManUse(char *kernalName, int partitionID, \name_t *arr, void (*\funcPtrUse)( ... ))&  Register user function to \funcPtrUse.\\
%		%		\hline
%		%		void \funcRegisterManDef(char *kernalName, int partitionID, \name_t *arr, void (*\funcPtrDef)( ... )) &  Register user function to \funcPtrDef.\\			
%		%		\hline
%	\end{tabularx}
%	\label{tab:prototype}
%	\vspace{-20pt}
%\end{table*}

% Fig.~\ref{sf:sysB} shows the execution phase. The main tasks of the \name\ execution phase are (1) maintaining information about \name\ sections residing on hosts and in devices, (2) determining and scheduling communication to ensure up-to-date data is available for computations, and (3) launching kernel executions. 

\paragraph{\funcinit} initializes the MPI and OpenCL systems and reads in data generated by the frontend.
%to initialize the LDEF and LUSE sets.  
A table is maintained for each \name 's use in a kernel call, which is initialized with information gathered by the frontend from  \emph{use} and \emph{def}.  This use/def and partitioning information are used to generate inter-process and host-device communication.
%
%\Samcomment{deleted selective device discussions unless we need.  Can put in a one-liner that the capability exists be removed for brevity.}
% The selective device feature is implemented using \texttt{clGetDeviceInfo()} to find a unique device ID that the device information file specifies. The unique ID is a combination of the PCI bus and slot ID for each device. \Samcomment{Do we use this selective device stuff anywhere?  If not, we should delete it and just mention that it exists.}
The last parameter of the \funcinit~function provides a device information file containing tuples \emph{(MPI rank, device ID)} to the kernel.  Note that MPI rankfile allows the MPI rank to be known before a program run.
% The MPI rank can be fixed and known before the program runs using MPI rankfile, so the rank becomes the unique ID of each device.
The device ID can be used to specify which device(s) to use when multiple devices are available to a process. 

\paragraph{\funccreate} creates a host and device buffer for the \name\ on each process using \texttt{malloc()} and \texttt{clCreateBuffer()} respectively, and allocates and initializes the \name's GDEF.

\paragraph{\funcpartition} evenly partitions work item regions for each device for a given partitioning type. It then defines the partitioned work item region entry in a partition table 
%\Samcomment{update structures with this} 
maintained for the \name\ and return a unique partition ID that is used for work and data distribution.

\paragraph{\funcapplykernel} manages communication and launches a kernel.  It performs the following actions:
\begin{itemize}[leftmargin=*]
\item Bind arguments to the kernel call.  %Passes argument values to the OpenCL function \texttt{clSetKernelArg()}.  
The system finds the device buffer from \name\ handle, binds all other arguments directly, and calls the OpenCL function \texttt{clSetKernelArg()}.
\item Determine and perform communication.  {\em Use} \name s trigger communication. 
%LUSE is updated by composing offset for the use (in the kernel table) with partitioned work item regions, and the LUSE is intersected with GDEF to determine data to be received and sent and the communication pattern.
LUSE is updated by composing \emph{use} offset (in the kernel table) with partitioned work item regions, and the LUSE is intersected with GDEF to determine communication (Eqns.~\ref{eq:intersectionsend} and~\ref{eq:intersectionrecv}).  If the intersection resides in the device, it is transferred to the host using \texttt{clEnqueueReadBufferRect()}.
Then, any needed inter-process non-blocking (e.g., point-to-point or collective) communication is done, followed by transferring data to the device using \texttt{clEnqueueWriteBufferRect()}. 
%Finally, the system updates the GDEF sets, as described in Eqn.~\ref{eq:subtract_send} and~\ref{eq:subtract_recv}.
Finally, the system updates the GDEF sets, as described in Eqns.~\ref{eq:update_gdef_send} and~\ref{eq:update_gdef_recv}.

\begin{sloppypar}
\item Execute the kernel. The preferred work-group size is found using \texttt{clGetKernelWorkGroupInfo()}, the work-group size is set, and the kernel is called using \texttt{clEnqueueNDRangeKernel()}.  Modified device buffers are known because of the {\em def} offset from the kernel table, and  
%data written on the device is known, and is transferred from the device to the host.
%the system updates LDEF and GDEF (Eqn.~\ref{eq:union_send} and~\ref{eq:union_recv}) so that the host has the coherent copy.
the system updates LDEF and GDEF (Eqns.~\ref{eq:update_gdef_send} and~\ref{eq:update_gdef_recv}) so that the host has the coherent copy.
\end{sloppypar}
\end{itemize}

\paragraph{\funcabsuse~and \funcabsdef} specify the absolute sections of the \name s annotated with \emph{use@} or \emph{def@} clauses (Section~\ref{subs:clauses}) which are then used to define LUSE and LDEF for each device.  LDEF updates must be precise because they affect GDEF, which defines who owns the coherent copy of a value. 
Multiple \funcabsdef~calls can be used to give precise updates, but for ease of programming and avoiding errors in entering each absolute section, \name\ supports predefined shapes for absolute section updates for LDEF (and LUSE).  For example, the \functrapezoiddef~function supports LDEF updates for two-dimensional trapezoidal or triangular shapes, which avoids multiple \funcabsdef~calls to update the LDEF. 
%\Hyundokcomment{other optional APIs are commented out from Table~\ref{tab:prototype}} that return the partitioned region boundary information for each device, and that user can define callbacks for the absolute section updates. \Samcomment{What are these callback functions?  Do we mention them earlier?} \Hyundokcomment{No, these are APIs that commented out in Table 3. Users can define callbacks so that \funcabsuse, \funcabsdef, and \functrapezoid~can be called from user-defined functions; otherwise they need to call those functions right before the \funcapplykernel. I changed the sentence a little bit. Does this provide enough information?} \Hyundokcomment{And again, these is the sub-sub-section that I commented in Section~\ref{subs:clauses} ("\emph{Absolute Section Interface Clauses:} use@ and def@"). Should we have the new sub-section and show clauses and API all toghether?}
%can call \funcabsdef~function, line by line, to update non-rectangular shape LDEFs. More convenient way is using 

\paragraph{Utility library functions}
In addition to the core API functions, utility library functions are provided.  I/O utility functions allow the programmer to move data between user space arrays and \name s.  The \name\ runtime updates the GDEF, LDEF, and LUSE information to reflect the data movement, thus keeping these consistent with the actual memory state.  Reduction functions are also provided.  If all data for an \name\  is in the host memories, a local reduction followed by an MPI reduction is performed.  If some or all data is in the device memory, a device reduction is performed followed by an MPI reduction.

%\subsection{Multi-node Accelerator Resource Management}
%\label{subs:partition}
%The last parameter of the \funcinit~function provides a device information file containing tuples \emph{(MPI rank, device ID)} to the kernel.  Note that MPI rankfile allows the MPI rank to be know before a program runs.
%% The MPI rank can be fixed and known before the program runs using MPI rankfile, so the rank becomes the unique ID of each device.
%The ID can be used to specify which device(s) to use when multiple devices are available to a process. 

%%
%the last parameter of the \funcinit~function allows a device information file containing tuples (MPI rank, device ID) to the kernel. The MPI rank \Samcomment{this is defined at runtime by MPI init} can be fixed and known before the program runs, so the rank becomes the unique ID of each device. The runtime uses the user-preferred device and let users manage device resources and users also can look up the device ID and other information through the \funcshow~library function.
%
%\begin{lstlisting}[caption={Manually partitioned Correlation host code.},label={code:partition}, frame=lines, breaklines=true, xleftmargin=2em, framexleftmargin=1.5em, numbers=left, numberstyle=\tiny, numbersep=5pt, captionpos=b, float=htb, belowskip=-2em, aboveskip=-1em,  basicstyle=\tiny]
%  ...
%#pragma hdarray partition(part0,        (10240,10240),\
%                          dev:0,   (0,3008),(0,10240),\  
%                          dev:1,(3008,7232),(0,10240))
%  ...
%  HDArrayApplyKernel("corr_ker1", part0, ... );
%  HDArrayApplyKernel("corr_ker2", part0, ... );
%  ...
%\end{lstlisting}
%%
%The \name\ interface also lets users partition arrays at any program point using the \emph{partition} clause shown in Table~\ref{tab:clauses}. Listing~\ref{code:partition} shows the manual definition of a partition specifying regions of the array assigned to each process in the {\tt hdarray} pragma.  In the two \funcapplykernel\ calls, the paritition is used to determine the work distributions of the two kernels. This is beneficial because different kernels may need different work distribution for load balancing of work across devices, or using a partial devices when this is more efficient than communicating the data. Although manual partitioning requires understanding of the communication patterns of the kernels, it gives more control and flexibility to programmers.  

\subsection{A Case Study: Matrix Multiply}
\label{subs:usecase}

Listing~\ref{code:host} and~\ref{code:device} show a General Matrix Multiply (GEMM) implemented using \name. The program uses C host code and OpenCL device code to perform the matrix multiply $C = A\times B$ on three 1024$\times$1024 2D matrices.

\begin{lstlisting}[	caption={GEMM host code.},label={code:host}, frame=lines, breaklines=true, xleftmargin=2em, framexleftmargin=1.5em, numbers=left, numberstyle=\tiny, numbersep=5pt, captionpos=b, float=htb, aboveskip=0em, belowskip=-2em]
void main(int argc, char *argv[]) {
  int ni = 1024, nj = 1024, nk = 1024;
  float a[ni][nk], b[nk][nj], c[ni][nj], alpha, beta;
  ... // initialize variables
  
  HDArrayInit(argc, argv, "gemm.cl", NULL);
  int part0 = HDArrayPartition(ROW, 2, ni, nj, 0, 0, ni, nj)
  
  HDArray_t *hA = HDArrayCreate("a", "float", a, 2, ni, nk);
  HDArray_t *hB = HDArrayCreate("b", "float", b, 2, nk, nj);
  HDArray_t *hC = HDArrayCreate("c", "float", c, 2, ni, nj);
  HDArrayWrite(hA, a, part0);
  HDArrayWrite(hB, b, part0);
  HDArrayWrite(hC, c, part0);
  
  HDArrayApplyKernel("gemm", part0, hA, hB, hC, alpha, beta, ni, nj, nk);    
  HDArrayRead(hC, c, part0);
  HDArrayExit();
}
\end{lstlisting}
%
\begin{lstlisting}[caption={GEMM device code.},label={code:device},frame=lines, breaklines=true, xleftmargin=2em, framexleftmargin=2em, numbers=left, numberstyle=\tiny, numbersep=5pt,	literate={_}{\textsmallunderscore}1, captionpos=b, float=htb, belowskip=-3.5em] 
#pragma hdarray use(A,(0,*)) use(B,(*,0)) def(C,(0,0))
__kernel void gemm(__global float *A, __global float *B, __global float *C, 
                   float alph, float beta, int ni, int nj, int nk) {
  int i = get_global_id(1), j = get_global_id(0);
  if ((i < ni) && (j < nj)) {	
     C[i * nj + j] *= beta;
     for(int k=0; k < nk; k++)
        C[i*nj+j] += alph * A[i*nk+k] * B[k*nj+j];
  }
}
\end{lstlisting}
%
%The host code in Listing~\ref{code:host} initializes variables and the system, generates the \emph{partition ID} used for data and work partitioning, registers user program arrays with the \name s, invokes the kernel with arguments, writes/reads arrays to/from the accelerator devices, and closes down the system.

Line 6 of the host code initializes the MPI and OpenCL environments and finds available devices to run the OpenCL kernel implemented in ``{\tt gemm.cl}''. 
Line 7 evenly partitions the highest dimension of 2D array domain with regards to the number of devices. The function returns a partition ID, {\tt part0}, which represents the partitioned region and is used throughout the program. 

On lines 9-11, the host creates \name s and allocates host and device buffers with the same size of user-space arrays. 
After the allocation, the host binds program array variables ({\tt a}, {\tt b}, {\tt c}) to handles ({\tt hA}, {\tt hB}, {\tt hC}) that point into structures in the \name\ runtime and allow users to access device buffers holding data for their respective program arrays.
Lines 12-14 write user arrays into the device buffer of \name s according to the {\tt part0} specification. Therefore, the data is distributed to different devices.

On line 16, the host launches the ``gemm'' kernel using the {\tt part0} and kernel arguments. {\tt part0} is used for work distribution. As shown in Fig.~\ref{fig:applykernel}, the runtime then binds \name\ handles and host variables to the kernel arguments, handles necessary communication, and invokes the kernel (Listing~\ref{code:device}).
%%
%Line 17 retrieves the result of the computation from the device memory and moves it into user array {\tt c}. Similar to the \funcwrite\ call, the \funcread\ call uses {\tt part0} to read each portion of the distributed array {\tt hC} into user array {\tt c}. 
Line 17, reads the result of the computation from the device memory into user array {\tt c}. 
Finally, the host frees all the resources, including \name 's, and finalizes the parallel program in line 18. 
%

The device code in Listing~\ref{code:device} shows an ordinary OpenCL kernel to be called, with an annotation added on line 1. The annotation is a {\tt \#pragma \MakeLowercase{\name}} statement with offset clauses discussed in Section~\ref{subs:clauses}. These offsets, relative to a work item index, specify slices of the {\tt A}, {\tt B}, and {\tt C} arrays that are used and defined.
%Hereafter, we use the terms work item and thread interchangeably. 
The code informs the runtime system that a single thread reads all elements of the row of the array {\tt A} and all elements of the column of the array {\tt B}. The zero offset indicates that each thread writes the result of the multiplication to its work item index of the array {\tt C}.

With the work partitioning ({\tt part0}) and per-thread array element access (offset) information provided by the host and device code, respectively, the runtime is able to generate LUSE and LDEF, and distribute work for the kernel.


==> arxiv_hdarray/eval.tex <==
In this section, we evaluate the effectiveness of the proposed techniques with six publicly available benchmarks. 
% We compare the scalability of the system's automatic distribution with manual distribution to show how users can reduce communication cost by using the \name\ interface. The speedup versus serial version is presented, followed by a discussion of the overhead of the runtime system. In addition, we provide the evaluation of the communication trend for each benchmarks, running on the runtime system. \Hyundokcomment{what is the main point of evaluating communication trend?}
%
%\subsection{Experimental Setup}
%\label{subs:exp_setup}
Our evaluation is done using up to 32 OpenCL devices (limited by Xsede job submission policies) on the Xsede Comet cluster~\cite{towns2014xsede,Moore:2014:GDC:2616498.2616540}. Comet has 1,944 compute nodes and 72 GPU nodes, connected by a 56 Gbps FDR Infiniband. Each compute node consists of two 12 core Intel Xeon CPU E5-2680 processors running at 2.50 GHz, 128 GB of main memory. The GPU nodes consist of 36 NVIDIA P100 nodes and 36 NVIDIA K80 nodes, and each node has 4 GPUs. We use both P100 and K80 GPU nodes, each of which has total 40GB of device memory and utilize 4 GPU devices per node.

We use six micro-kernel benchmarks: GEMM, 2MM, 2D Convolution, Jacobi, Covariance, and Correlation from the Polyhedral Benchmark Suite for GPUs and accelerators (PolyBench/ACC)~\cite{6339595}.  We compile the benchmarks with gcc 4.9.2 with -O3 and use OpenMPI version 1.8.4. OpenCL version 1.2 is used to support NVIDIA devices.  Baseline numbers are found using the implementations provided by the benchmarks.  For \name\ system numbers, the OpenCL device code is augmented with \name\ pragmas with \emph{use} and \emph{def} clauses, and C host code that includes \name\ library calls and \emph{partition} clauses are added.
%
% RINK
%Our evaluation utilizes up to 8 nodes with 4 GPU devices per node. 

\begin{figure*}[t]
	\centering
%	\vspace{-15pt}
%	\subfloat{\includegraphics[width=4.8in]{fig/scalability2}}%
%	\subfloat{\includegraphics[max width=\textwidth]{fig/scalability2}}%
	\subfloat{\includegraphics[width=4.5in]{fig/scalability3base}}%
%	\subfloat{\includegraphics[max width=\textwidth]{fig/scalability3base}}%
	\vspace{-10pt}
	\caption{Scalability for the \name\ runtime system on P100 and K80 nodes. We show the speedup for each benchmark, which is the ratio of the execution time of a single device to the execution time of the number of devices indicated on the x-axis. All the benchmarks use an automatic row-wise partitioning for data and work distribution.}
	\label{fig:eval_scalability}
	\vspace{-15pt}
\end{figure*}

\subsection{Scalability}
\label{subs:eval_scalability}
%
%\begin{figure*}[!htb]
%	\centering
%	\subfloat{\includegraphics[width=7.1in]{fig/scalability}}%
%	\vspace{-5pt}
%	\caption{Scalability for the \name\ runtime system with different partitioning methods. We show the speedup for each benchmark, which is the ratio of the execution time of a single device to the execution time of the number of devices indicated on the x-axis.}
%	\label{fig:eval_scalability}
%	\vspace{-15pt}
%\end{figure*}
%
Fig.~\ref{fig:eval_scalability} shows strong scaling on both P100 and K80 nodes. The baseline time is for running one OpenCL device without \name.  All the benchmarks perform a row-wise partition using the \funcpartition~function with a ROW argument for work and data distribution. Most benchmarks running on K80 nodes scale better than on P100 nodes because the P100 is faster than the K80, and thus the communication overhead on P100 nodes is a larger fraction of the computation time. 
%while communication time is the same. Therefore, the communication overhead has a bigger impact on the scalability in P100 nodes.


%We use 8 nodes with up to four devices per node, with additional nodes added only after four processes are executing on a node. 

GEMM, shown in Section~\ref{subs:usecase}, uses 10,240$\times$10,240 matrices with 100 iterations. The \name\ runtime system detects and generates all-gather collective communication because each OpenCL work-item needs row and column elements of arrays for computation. Scaling is good to 32 processes, with similar efficiencies on the K80 (92\%) and P100 (90\%), due to the low ratio of communication to kernel execution time.
2MM performs two matrix multiplications, $D = A \times B$ followed by $E = C \times D$. It differs from GEMM in that 2MM runs two kernel functions within a loop and exhibits a data dependency because one kernel defines the array $D$ used by the other kernel. With the row-wise partitioning, the efficiency drops off to about 75\% (42\%) on the K80 (P100) at 32 processes because of the communication cost. The cost is proportional to the number of processes, and every iteration requires the communication: once for the array $B$, and 100 times for the array $D$.   % \Samcomment{It's really proportional the number of processes or number of columns, isn't it?} \Hyundokcomment{The number of iteration affects the number of communication and the cost for each communication is proportional to the number of processes. Updated.}

A different partitioning can be used to reduce the communication cost. 2MM with column-wise partitioning, as shown in Fig.~\ref{fig:scalability_diff_partition}, only communicates twice for arrays $A$ and $C$, and the efficiency is about 98\% (96\%) on the K80 (P100) at 32 processes. Table~\ref{tab:partitioning} shows communication volumes of all 32 processes and noticeable volume difference for 2MM.  This performance tuning was done by simply changing the \partitiontype\ argument of \funcpartition~function.

\begin{figure*}[t]
	\centering
%		\vspace{-15pt}
	\subfloat{\includegraphics[width=3.2in]{fig/partitioncompbase}}%
	%	\subfloat{\includegraphics[max width=\textwidth]{fig/partitioncomp}}%
	\vspace{-10pt}
	\caption{Scalability for the \name\ runtime system with different partitioning methods. 2MM uses automatic column-wise partitioning and Correlation uses manual row- and column-wise partitionings.}
	\label{fig:scalability_diff_partition}
%	\vspace{-5pt}
\end{figure*}
%
\begin{table}[t]
	\scriptsize
	\renewcommand{\arraystretch}{1.3}
%	\vspace{-8pt}
	\centering
	\caption{Total communication volume for 32 processes}
	\label{tab:partitioning}
	\vspace{-8pt}
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		Partition & Convolution   & JACOBI       & GEMM     & 2MM          & Covariance & Correlation \\
		\hline
		Default (Row)        & 5 MB                & 473 GB        & 12  GB     & 1262 GB    &  1268 GB     &  1268 GB      \\
		Customized  & 5 MB                & 473 GB         & 12 GB     & 25 GB        &  811 GB     &   811 GB      \\
		\hline
	\end{tabular}
	\vspace{-15pt}
\end{table}
%

Both Jacobi and Convolution kernels are iterative stencil codes, with four and eight neighbors, respectively.  The offsets of \emph{use} and \emph{def} clauses have similar patterns for both benchmarks. For Jacobi, the device code consists of two kernels. One kernel processes the following computation: 
{
\small
\begin{align*}
A[i][j]=(B[i][j-1]+B[i][j+1]+B[i-1][j]+B[i+1][j]) / 4
\end{align*}
%\vspace{-0.25em}
}%
%~\footnote{For the illustration purpose, a regular C code is used.}
The \emph{use} clauses are specified for the kernel with four offsets, (0,-1), (0,+1), (-1,0), (+1,0), for an array $B$. The other kernel performs $B[i][j]=A[i][j]$, and zero offsets are used. The host code allocates user space arrays to have ghost cells at the array boundary, and then generates two partition IDs: one that partitions the entire region for data distribution and the other that excludes the cells for work distribution. Two kernels have a data dependency on array $B$ in the iteration space. Convolution has four additional offsets added, but there is no data dependency. Both kernels use 20,480$\times$24,080 matrices with 100,000 iterations, and the runtime detects and schedules a point-to-point communication. 
%Since using a 2D block partitioning increased the number of messages and communication cost, we utilize a column-wise manual partitioning to contrast with the automatic row-wise partitioning. 
Both benchmarks scale well with an efficiency of 88\% (68\%) on the K80 (P100) for Jacobi, and 91\% (93\%) on the K80 (P100) for Convolution at 32 processes. Similar to GEMM, two nodes for Convolution show similar efficiencies due to the small communication overhead.
%Scaling is poor because of \name\ runtime system overhead (discussed in Section~\ref{subs:eval_overhead}), not only communication overhead. 
%Scaling is poor primarily because of \name\ runtime system overhead, not communication overhead. 
%
%

Covariance and Correlation are data mining benchmarks that compute a measure from statistics that show how linearly related two variables are. These benchmarks have triangular-shape array accesses, requiring the absolute section interface discussed in Section~\ref{subs:absclause}.
Both use 10,240 vectors and 10,240$\times$10,240 matrices with 100 iterations, and the system detects point-to-point and all-gather communication. 
%The most time consuming kernels of these benchmarks have triangular-shape array accesses which utilize up to 50\% of device resources and require the absolute section interface discussed in Section~\ref{subs:absclause}. 
Scaling is poor with the default row-wise partitioning with an efficiency of 27\% (16\%) on the K80 (P100) for Correlation (similar to Covariance).
%due to the work and communication imbalances. This is because \funcpartition~evenly divides work item regions with the number of devices and the most computation uses the upper-triangular sections only, and later make the array symmetric by copying upper-triangular to lower-triangular sections. 
This is because evenly distributing work using \funcpartition~causes poor work and communication load balancing for kernels that have triangular access patterns. The most time-consuming computation is done from the upper-triangular section of an array which later requires communication to make the array symmetric. As a result, each device gets a different amount of work, and a device with the most computation also has the most communication, which leads to the imbalance of computation and communication across the devices.
%\Hyundokcomment{I got better result with different manual partitioning and absolute section update. Previous result was 36\% (19\%) and now it's 43\% (25\%). Also updated this paragraph since the improvement comes from both communication and work balancing.} 

Manual partitioning (Listing~\ref{code:partition}) with optimized absolute section updates to balance the work and communication among devices, gives better scalability with an efficiency of 44\% (24\%) on the K80 (P100) with the reduced communication volume as shown in Fig.~\ref{fig:scalability_diff_partition} and Table~\ref{tab:partitioning}, respectively. This result highlights the value of integrating manual and automatic partitioning.
% %Table~\ref{tab:partitioning} shows no difference in communication volume for two different partitionings, but the work balancing helps. 
Also, the performance tuning does not require any changes in kernel code, but only a few lines are changed in absolute section updates and partitioning in  the host code.

\subsection{Runtime Overhead}
\label{subs:eval_overhead}

\begin{figure}[tb]
	\centering
	%	\vspace{-15pt}
%	\includegraphics[width=4.3in]{fig/overheadall}
	\includegraphics[width=4in]{fig/overheadall2}
	%	\includegraphics[max width=\textwidth]{fig/overheadall}
	\vspace{-10pt}
	\caption{Total runtime overhead for all six benchmarks on both P100 and K80. The highest overhead is 0.35\% from Jacobi on P100.}
	\label{fig:overheadall}
	\vspace{-10pt}
\end{figure}
%
\begin{figure}[tb]
	\centering
	%	\vspace{-25pt}
	\includegraphics[width=4in]{fig/overheadjacobi3}
	%	\includegraphics[max width=\textwidth]{fig/overheadjacobi2}
	\vspace{-10pt}
	\caption{Breakdown of runtime overhead for Jacobi on P100. There is no overhead of GDEF updates  because these updates are overlapped with communication and computation. Running a single device also does not incur any overhead.}
	\label{fig:jacobi_overhead}
	\vspace{-13pt}
\end{figure}

% The runtime system shows acceptable overhead up to 32 processes. 

%Fig.~\ref{fig:overheadall} shows the percentage of runtime overhead for all six benchmarks on both P100 and k80, based on total execution time. All of the benchmarks have less than 0.36\% overhead. 
%The highest overhead comes from Jacobi running on the P100, and Fig.~\ref{fig:jacobi_overhead} shows the rate and time of each runtime component's overhead. 
%
%Breaking down the overhead of Jacobi on P100, the overhead of GDEF updates are zero because they overlap with, and finish before, the communication and kernel computation.
%The LDEF and LUSE update overhead does not linearly increase in time because the local sections are reused after the first iteration. 
%The intersection overhead, which includes both intersection time and caching (Section~\ref{subs:optimization}) time, showed the largest overhead (0.25\% out of 0.35\%), mainly due to the caching. While not shown in the graph, the overhead of intersection without caching is about 4.7\%, which is 19 times larger than with caching enabled. 
%However, the caching overhead for Jacobi is higher than other benchmarks because the runtime creates many LDEF-LUSE chains of history buffer, and the time for tracking the chains takes a larger portion of total execution time than the other benchmarks. Jacobi also has fragmented GDEF sections, requiring more GDEF comparisons than all other benchmarks. The system reduces the number of GDEF, LDEF, and LUSE sections for other benchmarks by merging adjacent or redundant sections, but the fragmented sections cannot be merged.  

Fig.~\ref{fig:overheadall} shows the percentage of runtime overhead based on total execution time. All of the benchmarks have less than 0.36\% overhead on up to 32 processes. The benchmarks on a P100 node have more overhead than on a K80 as the P100 is faster than the K80, similar to the scalability difference. Our effort to minimize the runtime overhead, as discussed in Section~\ref{subs:optimization}, significantly reduced the cost of calculating GDEF, LDEF, LUSE, and intersection for all the benchmarks. Without the optimization, the \name\ baseline system suffers from the overhead of section calculations, which increases proportional to the number of processes.

Breaking down the highest overhead benchmark in Fig.~\ref{fig:jacobi_overhead}, the overhead of GDEF updates are zero because they overlap with, and finish before, the communication and kernel computation. This is a large improvement because every kernel call requires the GDEF update.
The intersection overhead, which includes both intersection time and caching time, is much smaller, e.g., by a factor of 19 for Jacobi on P100, than the baseline system. The result shows the benefit of using the LDEF/LUSE history buffer and linear-time GDEF comparison. 
Caching LDEF and LUSE for each kernel call is also beneficial. The LDEF and LUSE update overhead does not linearly increase in time because the local sections are reused after the first iteration of the kernel call. 
Finally, although not shown in the figure, the system reduces the number of sections by merging adjacent or redundant sections, further reducing the overheads of intersecting.

%
%
%\begin{table}[ht]
%	\renewcommand{\arraystretch}{1.3}
%	\centering
%	\vspace{-5pt}
%	\caption{Runtime overhead of Jacobi as a percentage of total execution time: caching disabled and enabled}
%	\label{tab:overhead}
%	\vspace{-5pt}
%	\begin{tabular}{|c|c|c|c|c|c|}
%		\hline
%		Number of Processes & 2 & 4 & 8 & 16 & 32 \\
%		\hline
%		No Caching  & 0.261 & 0.779 & 2.147 & 5.539 & 14.120 \\
%		Caching  & 0.109 & 0.351 & 0.923 & 2.882 & 8.472 \\
%		\hline
%	\end{tabular}
%	\vspace{-5pt}
%\end{table}
%
%
%
%The \name\ system's largest runtime overhead is performing intersections. Table~\ref{tab:overhead} shows that the overhead is reduced by the caching strategy of~Section~\ref{subs:caching}. 
%\Hyundokcomment{Do we need to mention more details about Table~\ref{tab:overheadnocache} and ~\ref{tab:overhead}, e.g., what the percentage represents, explain the highest improvement, Jacobi?} ~\Hyundokcomment{Also, does Table~\ref{tab:overheadnocache} and ~\ref{tab:overhead} look good? Or should I make those to one bigger table or concatenate Table~\ref{tab:overhead} to Table~\ref{tab:overheadnocache}?}
%Other overheads are primarily from LDEF, LUSE, and GDEF computations, which linearly increase as the number of processes increases. Both Convolution and Jacobi suffer from the overhead because the runtime generates many LUSE sections. Worse, the runtime updates and clears LUSEs and LDEFs for each kernel invocation, as shown in Algorithm~\ref{alg:applykernel}.
%\begin{table}[ht]
%	\renewcommand{\arraystretch}{1.3}
%	\centering
%	%	\vspace{-5pt}
%	\caption{Runtime Overhead of Jacobi as a Percentage of Total Execution Time: Caching Disabled and Enabled}
%	\label{tab:overhead}
%	%	\vspace{-5pt}
%	\begin{tabular}{|c|c|c|c|c|}
%		\hline
%		Number of Processes & No Caching & Caching\\
%		\hline
%		2 & 0.261 & 0.109\\
%		4 & 0.779 & 0.351\\
%		8 & 2.147 & 0.923\\
%		16 & 5.539 & 2.882\\
%		32 & 14.120 & 8.472\\
%		\hline
%	\end{tabular}
%	%	\vspace{-12pt}
%\end{table}
%
%Another reason for the overhead is managing section fragmentations when doing GDEF calculation. The \name\ runtime maintains precise GDEF sections for handling communication, which for Convolution and Jacobi results in many small sections because small portions of the array are communicated, and the messages are subtracted from GDEF (Eqn.~\ref{eq:subtract}). The small fragments would be communicated as individual messages, resulting in communication and data transfer overhead; however, the \name\ runtime system tries to merge the fragmented sections when a section is updated. This is a complex task because the system must consider both the host and device address spaces. Conservatively merging sections is possible only if those sections are in the same memory; if not, then additional work is required and even more fragmentation may occur.
%

%The highest overhead, 0.25\%, comes from Jacobi running on the P100 and is mainly due to the overhead of caching intersections, described in Section~\ref{subs:optimization}, as well as intersection time.  While not shown in the graph, the overhead of intersection without the caching is about 4.7\% which is 19 times larger than with caching enabled.  The LDEF and LUSE update overhead does not linearly increase in time because the local sections are reused after the first iteration.  The overheads of GDEF updates are zero because the updates overlap with, and finish before, the communication and kernel computation.  These overheads are high in Jacobi are because the runtime creates many LDEF-LUSE chains of history buffer, and the time for tracking the chains takes a larger portion of total execution time than in the other benchmarks.  Jacobi also has fragmented GDEF sections, requiring more GDEF comparisons than all other benchmarks.  The system reduces the number of GDEF, LDEF, and LUSE sections for other benchmarks by merging adjacent or redundant sections, but the fragmented sections cannot be merged.  

%The highest overhead comes from Jacobi running on the P100 mainly due to the overhead of caching intersections, described in Section~\ref{subs:optimization}. With Jacobi, the runtime creates many LDEF-LUSE chains of history buffer, and the time for tracking the chains takes a larger portion of total execution time than the other benchmarks. It also has fragmented GDEF sections, requiring more GDEF comparisons than all other benchmarks. The system reduces the number of GDEF, LDEF, and LUSE sections for other benchmarks by merging adjacent or redundant sections, but the fragmented sections cannot be merged.  
%Fig.~\ref{fig:jacobi_overhead} shows the rate and time of each runtime component's overhead for Jacobi. The highest overhead, 0.25\%, comes from intersection and includes both the intersection time and the caching overhead. While not shown in the graph, the overhead of intersection without the caching is about 4.7\% which is 19 times larger than with caching enabled. The LDEF and LUSE update overhead does not linearly increase in time because the local sections are reused after the first iteration. The overheads of GDEF updates are zero because the updates overlap with, and finish before, the communication and kernel computation.

%Improving the scalability of the \name\ runtime is part of our ongoing work. One opportunity is to expand our caching techniques to the section updates. The system already avoids unnecessary intersections by caching each \name 's intersection history for each kernel, and the system at this point has enough information to skip unnecessary section updates.

% We now evaluate the communication characteristics for each benchmarks to compare communication costs on different network setup and show \name\ runtime's communication pattern detection and execution. Fig.~\ref{fig:eval_commtrend} shows average communication time among processes.  

% We use two different process-node configurations: 2 processes per node and 4 processes per node. This configuration shows different communication costs between inter-node and intra-node communication. Note that ethernet, in addition to infiniband, is used because 56 Gbps infiniband supports transport offload with Remote Direct Memory Access (RDMA), making little or no difference between inter- and intra-node communication. GEMM and 2MM use 7680$\times$7680 Matrices with 100 iterations and Convolution and Jacobi have 15360$\times$15360 Matrices with 100,000 iterations.

% GEMM and 2MM show that inter-node communication (2 per node) usually has penalty over intra-node communication (4 per node) although inter-node communiation in tcp network for GEMM fluctuates over 8 processes and inter-node communication in infiniband for 2MM outperforms intra-node communication. Both kernels need all-gather communication and the \name\ system detect the pattern by comparing LUSE with \name 's dimensions. Both kernels' communication cost linearly increase as number of processes increase as the system executes blocking MPI\_Allgatherv and we have more number of smaller messages to communicate.

% Convolution shows a lot of network noise almost impossible to analyze the result. This is because the message size is small and it communicates only once. Jacobi shows inter-node communication cost is higher than intra-node communication on both ethernet and infiniband network. The \name\ system detects the ptp communication pattern by intersecting LUSE with neighbor MPI processes and executes asynchronous MPI\_Isend and MPI\_Irecv. \Hyundokcomment{is it too long? should I delete the following lines?}The results shows penalty from 2 to 4 processes which is due to partitioning method and device data transfers. From 4 processes and more, the first and last process get half messages, compare to other processes, and data transfer time varies process to process, which makes the first and last process wait longer than others.

%\begin{figure}[!t]
%	\centering
%	\begin{subfigure}%{0.5\textwidth}
%		\centering
%		\includegraphics[width=1.5\linewidth]{fig/commtrend2MM}
%		\caption{2MM Results}
%		\label{fig:eval_commtrend_2mm}
%	\end{subfigure}%
%	\begin{subfigure}%{0.5\textwidth}
%		\centering
%		\includegraphics[width=1.5\linewidth]{fig/commtrendJacobi}
%		\caption{Jacobi results}
%		\label{fig:eval_commtrend_jacobi}
%	\end{subfigure}
%	\caption{filler text}
%	\label{fig:eval_commtrend}
%\end{figure}

%\begin{figure*}[!t]
%	\centering
% 	\subfloat{\includegraphics[width=7.1in]{fig/commtrend}}%
% 	\caption{Communication Trend for each benchmarks comparing the cost of intra-node (2 devices per node) communication with inter-node (4 devices per node) communication on ethernet (tcp) and infiniband (inf) network}
% 	\label{fig:eval_commtrend}
% \end{figure*}

%\subsection{Accelerator Utilization}
%\label{subs:eval_hydrid}


==> arxiv_hdarray/implemention.tex <==
This section describes some implementation details not covered in Section~\ref{subs:ui}.  

 \subsection{Frontend and Execution Phase}
\label{subs:front_exec_phase}
% \subsection{Frontend Phase}
% \label{subs:setup}

 The frontend phase, shown in Fig.~\ref{sf:sysA}, uses a simple parser that performs three tasks: (1) parse OpenCL kernel functions and \name\ pragmas, (2) collect information, including {\em use} and {\em def} offset information, that is written to the file $ M $ (Fig.~\ref{fig:overview}) used to initialize the \name\ table, and (3) generate code for \name\ pragmas and directives that pass partitioning information to the runtime.
%
% If the frontend phase encounters manual partitioning directives, as discussed in Section~\ref{subs:partition}, the parser expresses the directives as calls to internal \name\ runtime routines. The call is essentially same as \funcpartition\ and returns partition ID to the variable defined in the \emph{partition} clause. Because the information is passed at runtime, variables can be used to specify regions, etc., and their value will be used to update GDEF, LDEF, and LUSE.
%
%\subsection{Execution Phase}
%\label{subs:executinphase}

Fig.~\ref{sf:sysB} shows the execution phase. The main tasks of the \name\ execution phase are (1) maintaining information about \name\ sections residing on hosts and in devices, (2) determining and scheduling communication to ensure up-to-date data is available for computations, and (3) launching kernel executions.  
%Algorithm~\ref{alg:applykernel} sketches the logic of \funcapplykernel~which is the core part of the execution phase.
Fig.~\ref{fig:applykernel} sketches the logic of \funcapplykernel~which is the core part of the execution phase. 
%\Samcomment{I commented out \name\ also provides helper functions \ldots.} % \name\ also provides helper functions (Table~\ref{tab:prototype}) that user can define callbacks for the absolute section interface APIs discussed in Section~\ref{ssub:api}, which simplifies the absolute section updates.
%
%%\vspace{-5pt}
%\setlength{\textfloatsep}{5pt}% Remove \textfloatsep
%\begin{algorithm}[ht]
%	\caption{Pseudo code of \funcapplykernel}
%	\label{alg:applykernel}
%	\tiny
%	\begin{algorithmic}[1]
%		\Procedure{\funcapplykernel}{kernel name, region, arguments}
%		\State get kernel ID from kernel table
%		\State set kernel arguments
%		\For{each $\name$ in kernel arguments}
%		\If{type of $\name$ is USE}
%		\State update LUSE
%		\State detect and schedule communication					
%		\If{scheduled}
%		\State data transfer from device to host
%		\State execute communication
%		\State data transfer from host to device
%		\State update GDEF (subtraction)
%		\EndIf
%		\EndIf 
%		\EndFor
%		
%		\State kernel execution
%		
%		\For{each $\name$ in kernel arguments}
%		\If{type of $\name$ is DEF}
%		\State update LDEF
%		\State update GDEF (union)
%		\EndIf 
%		\State clear LDEF and LUSE
%		\EndFor
%		\EndProcedure
%	\end{algorithmic}
%\end{algorithm}
%% \vspace{-5pt}
%
\begin{figure*}[htb]
	\centering
	\vspace{-15pt}
%	\subfloat{\includegraphics[max width=\textwidth]{fig/applykernel}}%
	\subfloat{\includegraphics[width=4in]{fig/applykernel}}%
	\vspace{-10pt}
	\caption{Logic of \funcapplykernel~function.}
	\label{fig:applykernel}
	\vspace{-30pt}
\end{figure*}
%
% \subsection{Discussion: Improving Runtime Overhead}
%\label{subs:caching}
%
% A major runtime overhead comes from computing the intersections to perform communication. If the LUSE and GDEF for a kernel call are unchanged from the last call, the intersection from the last call can be used. If \emph{use} and \emph{def} for a kernel call is constant and the intersection is unchanged, it can be shown that the intersection will never change unless an \name\ is repartitioned. When an \name\ is repartitioned, all LUSE, GDEF, and intersections involving the array are set to NULL, forcing their re-computation. Our system uses this optimization to improve performance.

\subsection{Reducing Runtime Overhead}
\label{subs:optimization}

The major overhead incurred by our baseline runtime system comes from intersecting and updating array sections to determine communication. Data to send or receive are found by intersecting GDEF with LUSE sets, as shown in Eqns.~\ref{eq:intersectionsend} and~\ref{eq:intersectionrecv}, which requires the number of computations on each process $ p $ that is linear in the number of processes.
%Determining what array sections  process $ p $ will receive requires intersecting the LUSE for the $ p $ with $ p $'s GDEF RECV for all other processes. Similarly, for $ p $ to determine what sections to send requires intersecting the LUSE sets for all other processes with $ p $'s GDEF SEND. These intersections require computations on each $ p $ that is linear in the number of processes. 
To reduce the overhead, the \name\ system attempts to evaluate the intersections only when it is necessary to do so.  To assist in this, the system caches the last GDEF, LDEF, and LUSE sets as well as intersections per kernel call/partition ID. 
If LUSE and GDEF are unchanged for repeated kernel calls with the same partition ID, the system reuses the intersections from the last kernel call. 

%If the use and def information for a kernel call is constant and the intersection is unchanged, it can be shown that the intersection will never change unless the kernel uses a different work partitioning. When a new partition ID is used, the runtime creates LUSE and intersection involving the array. 
%
%\Hyundokcomment{I commented out the sentences starting with "For an ... " and updated the following paragraph. The previous paragraph says that we reuse cached intersections if GDEF and LUSE are not changed. In the following paragraph says why we need GDEF and LUSE comparisons and how we efficiently do the comparisons because the comparisons themselves incur overhead. And that is maintaining and evaluating a LDEF/LUSE ID history buffer. There are several different conditions for the evaulation, and we wanted to summarize those conditions. Instead of using "flow dependence", I used "use-def chain" to describe the evaulation in high-level and give one example of the evaluation (comparing two pairs of LDEF and LUSE IDs). Please check the paragraph. }
%For an array $ h $ that is defined in a kernel, the LUSE and LDEF sets can be used to determine if there is a flow dependence from the previous update.  If not dependence exists, communication is not necessary, and no intersection is needed.
%
%For an \name\ $ h $ that is read, its 
%
LUSE and LDEF sets, accessed in a repetitive kernel call with the same partition ID, can be reused.  However, GDEF sets for that kernel call can change as they are a function of the LUSE and LDEF sets \emph{and} all previous GDEFs. Therefore, the system must check whether the GDEF sets have changed.  
%
An exact comparison of GDEFs takes O($n^2$) time, but the GDEF comparison overhead is reduced in two steps. First, the system maintains history buffers of the IDs of LDEF and LUSE sets for each \name\ that tracks LDEF/LUSE IDs for the entire program. It then evaluates the def-use chains in the buffer to determine changes in GDEF. For example, the system compares the last LDEF and LUSE IDs with the current LDEF and LUSE IDs. If the two pairs are the same, GDEF sets for last and current kernels are also the same because a GDEF update is a function of LDEF and LUSE, thereby the system bypasses the GDEF comparison. %; otherwise, an O($n$) comparison of the sorted GDEF sections is done. 
%The evaluation of the history buffer, however, conservatively determines the changes, and it compares up to two pairs of LDEF/LUSE IDs. If a \name\ is defined and used in more than two kernels, the system gives up the evaluation. 
If the history buffer does not provide enough information, as the second step, the system performs an O($n$) comparison of GDEF sections, enabled by 
keeping the GDEF sections in sorted order when updated in Eqns.~\ref{eq:update_gdef_send} and~\ref{eq:update_gdef_recv}. The sorted GDEFs allow simple and linear-time GDEF comparisons.   

Finally, the system hides the overhead of section updates by overlapping the updates with host communication and device computation.  %It updates GDEF sets for \name~used (Eqns.~\ref{eq:subtract_send} and~\ref{eq:subtract_recv}) during the communication which are all non-blocking. The system also updates LDEF and GDEF sets for \name~defined (Eqns.~\ref{eq:union_send} and~\ref{eq:union_recv}) during the non-blocking kernel execution. 
It updates GDEF sets for \name~used during the communications which are all non-blocking. For a defined \name, the system updates LDEF and GDEF sets during the non-blocking kernel execution. 


==> arxiv_hdarray/intro.tex <==
%% no \IEEEPARstart
%% (should never be an issue)
%As GPU programming becomes more mainstream, both large and small scale multi-node systems with one or more GPUs per node have become common. However, these nodes complicate already messy distributed system programming by adding  MPI~\cite{gropp1999using} on top of proprietary host-GPU mechanisms. Developers must maintain two programming models: one for intra-process communication among devices and one for inter-process communication across address spaces.
%
%Proposed language extensions~\cite{kim2012snucl, kim2016distributed, gysi2016dcuda, kim2016impacc} support transparent access to accelerators on different nodes. Other library-based approaches~\cite{Chen:2012:PUA:2145816.2145838, vinas2016towards} provide high-level language abstractions and flexible array representations. These systems, however, require either low-level details of accelerator programming or explicit communication code. 
%In other systems~\cite{Lee:2011:EXP:2238356.2238410, potluri2013extending, 7081675}, programmers do not need to deal with the distribution of data,
%\Samcomment{Bu "implicitly expose" do we mean "expose communication details"?}
%\Hyundokcomment{"implicit" here means specifying affinity between data and thread (PGAS) mentioned in the first paragraph of Section~\ref{subs:related_acc_cluster}. This relieves programmers from dealing with data distribution. Updated the sentence.}
%but data is owned by a thread, leading to less flexible data and work distribution. Finally, compiler-assisted runtime systems~\cite{sakdhnagool2015hydra, Kwon:2012:HAO:2145816.2145827} translate and execute OpenMP programs on accelerator clusters, but the distribution of work and data are limited by OpenMP semantics and expressiveness.
%
%%To overcome the limitations of distribution options and static compiler information, we introduce the {\em \name} interface and runtime system. \name\ provides a programming model that abstracts away many of the details of programming multiple address spaces while allowing users to fine-tune the distribution of work and data among nodes and devices. \name\ programs use a global address space programming model. The system supports the automatic distribution of data across nodes, or the user can specify the distribution of arrays to aid in performance tuning. \name\ targets program execution on distributed systems whose nodes contain one or more accelerators. Parallelism is achieved using OpenCL~\cite{5457293} to create work on the {\em devices}, which, consistent with the OpenCL programming model, can be accelerators or cores. In our implementation, an MPI process or an OpenCL host matches a single OpenCL context and device.
%%
%%\name\ provides a runtime system, library, and annotations that allow high-level programming of heterogeneous distributed systems where nodes have accelerators (devices). Annotations are provided to distribute data across processes, or automatic partitioning can be used. Annotations also allow the specification of the data read, and written, during kernel invocations. The runtime automatically generates communication among nodes as well as from the host memory on a node to the device memory. Functions are also provided to allow selective reading of data on the device memory.
%%
%%To overcome the problem of needing multiple communication models to handle inter-node communication and communication between a node's host CPU and other devices on the node, \name\ supplies an API which, along with an underlying runtime library, provides a layer of abstraction for the different underlying communication models. To facilitate communication, the API allows the distribution of multi-dimensional arrays onto multi-node, distributed memory clusters. This solves the second problem in programming distributed heterogeneous machines, which is managing the actual communication operations. With the distribution, use and def information for individual nodes, global def information can be computed to efficiently manage both communications to/from different device memories in a process and among processes.
%
%The Heterogeneous Distributed Array ({\em \name}) interface and runtime system overcomes these limitations, 
%%\name\ programs use a global address space programming model with a library and annotations.
%targeting program execution on cluster-sized distributed systems whose nodes contain one or more accelerators. OpenCL~\cite{5457293} is used to create work on {\em devices}, either accelerators or cores.  
%\name\ APIs and annotations provide a global address space programming model to provide two benefits: 1) flexible distribution options and 2) high level abstractions of communication.
%%The model abstracts away many of the details of programming multiple address spaces while allowing users to fine-tune the distribution of work and data among devices in different nodes. 
%\name\ supports explicit and implicit data and work partitioning across devices, while overcoming the intrinsic limitations of static compilers~\cite{sakdhnagool2015hydra, Kwon:2012:HAO:2145816.2145827}. 
%%Different work partitioning and data distribution methods for computations are provided, e.g., kernels cam be launched with different work distributions. 
%Data can be distributed using \emph{offsets} relative to the data boundary of each OpenCL work item, thereby separating work partitioning from data distribution, allowing both work and data partitioning to be changed at any program point.  And, there is no data ownership, leading to flexible data and work distributions and addressing limitations of~\cite{Lee:2011:EXP:2238356.2238410, potluri2013extending, 7081675}. 
%\Samcomment{Should we mention these limitations?} \Hyundokcomment{Originally, we wanted to say how we overcome the limitations mentioned earlier. We need to discuss this because I'm not sure I understood your question.}
%
%As well, the \name\ API provides a layer of abstraction for the different underlying communication models. Annotations allow the specifications of the data read and written 
%during kernel invocations. The specifications also describe the offsets which can be easily derived from each kernel code. With distribution, use/def, and offset information, the \name\ runtime automatically generates efficient communication, overcoming the limitation of~\cite{kim2012snucl, kim2016distributed, gysi2016dcuda, kim2016impacc, Chen:2012:PUA:2145816.2145838, vinas2016towards}. The \name\ API and annotations relieve programmers from handling explicit communication, allowing them to focus on kernel programming.
%
%To summarize, our contributions are 
%\begin{enumerate}
%	\item An novel and easy programming model that can efficiently run on distributed heterogeneous devices and which separates work partitioning from data distribution, enabling flexible work and data distribution.
%	\item A fully automated intra-node and inter-node communication. 
%    % We describe a runtime communication generation scheme and present the implementation of the runtime system. 
%	\item A flexible user interface that allows manual tuning for high performance and works with the automatic communication. 
%    %The interface lets users utilize device resources to balance workloads and manually distribute data to reduce communication cost.
%	% \item A runtime system that is maintainable and extensible. We also discuss the overheads of the runtime system and opportunities for improvement.
%	\item Experimental results showing good performance and speedups on small clusters with eight nodes and 1 to 32 GPUs.
%\end{enumerate}
%
%% The rest of the paper is organized as follows. 
%Sections~\ref{s:design} and~\ref{s:impl} describe the design and implementation of the \name~interface. Section~\ref{s:eval} presents a performance evaluation of the \name~runtime system. Section~\ref{s:related} discusses related work, and conclusions and future work follow in Section~\ref{s:conclusion}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As GPU programming becomes more mainstream, both large and small scale multi-node systems  with one or more GPUs per node have become common. These nodes, however, complicate already messy distributed system programming by adding  MPI~\cite{gropp1999using} on top of proprietary host-GPU mechanisms. Developers must maintain two programming models: one for intra-process communication among devices and one for inter-process communication across address spaces.

%~\cite{kim2012snucl, kim2016distributed, gysi2016dcuda, kim2016impacc, Chen:2012:PUA:2145816.2145838, vinas2016towards} have been proposed to improve the programmability of multi-node systems with accelerators.
%
Several systems have improved the programmability of multi-node systems with accelerators. 
%Language extensions~\cite{kim2012snucl, kim2016distributed, gysi2016dcuda, kim2016impacc} support transparent access to accelerators on different nodes, and other library-based approaches~\cite{Chen:2012:PUA:2145816.2145838, vinas2016towards} provide high-level language abstractions and flexible array representations. 
%
%Language extensions (SnuCL~\cite{kim2012snucl, kim2016distributed}, dCuda~\cite{gysi2016dcuda}, and IMPACC~\cite{kim2016impacc}) support transparent access to accelerators on different nodes, and other library-based approaches (PARRAY~\cite{Chen:2012:PUA:2145816.2145838} and Vi{\~n}as \textit{et al}.~\cite{vinas2016towards}) provide high-level language abstractions and flexible array representations. 
%
SnuCL~\cite{kim2012snucl, kim2016distributed}, dCuda~\cite{gysi2016dcuda}, and IMPACC~\cite{kim2016impacc} support transparent access to accelerators on different nodes, and PARRAY~\cite{Chen:2012:PUA:2145816.2145838} and Vi{\~n}as \textit{et al}.~\cite{vinas2016towards} provide high-level language abstractions and flexible array representations. 
%
Programmers can develop high-performance applications but must manage low-level details of accelerator programming or provide explicit communication code. 
Partitioned Global Address Space (PGAS) platforms for accelerators, XMP-ACC~\cite{Lee:2011:EXP:2238356.2238410}, XACC~\cite{7081675}, and Potluri \textit{et al}.~\cite{potluri2013extending}, relieve programmers from dealing with data distribution, but data is strongly coupled to threads, making performance tuning more difficult. Finally, compiler-assisted runtime systems, Hydra~\cite{sakdhnagool2015hydra} and OMPD~\cite{ Kwon:2012:HAO:2145816.2145827}, propose a fully automatic approach that allows OpenMP programs to run on accelerator clusters, presenting an attractive alternative for developing repetitive, regular applications, but the distribution of work and data are limited by OpenMP semantics and expressiveness. 

% replacement text for the text below in the if(0)/\
In this paper, we describe the Heterogeneous Distributed Array (\name) interface and runtime system.  \name\ targets program execution on cluster-sized distributed systems with nodes containing one or more accelerators, i.e., devices.  Work is done as OpenCL work items, and \name\ provides ways to explicitly and implicitly partition work onto devices.  

\name\ also provides a way for the data used by the work on a device to be specified.  
The data read and written is typically relative to work items and can be specified either using offsets from the work item, or with an absolute specification of the data. 
\name\ then tracks the data defined and used by each work item, which allows communication to be generated automatically, since, in race-free programs, \name\ knows where the last written copy of a datum is, and who needs that value.  Importantly, data is not explicitly distributed and is not bound to, or owned by, a work item, but flows from its defining process and device to the process and device where it is needed.  
   
Finally, \name\ allows work to be repartitioned at any point in the program. This flexibility allows a programmer to optimize the work distribution and its necessary communication without any changes to the kernel code.
\if(0)
In this paper, we describe the Heterogeneous Distributed Array ({\em \name}) interface and runtime system that provides automatic communication and simple tuning for high performance.
%\name\ programs use a global address space programming model with a library and annotations.
\name\ targets program execution on cluster-sized distributed systems whose nodes contain one or more accelerators. OpenCL~\cite{5457293} is used to create work on {\em devices}, either accelerators or cores.  
\name\ APIs and annotations provide a global address space programming model to enable both automatic communication \Samcomment{is there a reason we don't say "automatic communication" instead of "high level abstractions of communication"?}\Hyundokcomment{Agree. We should say automatic. Updated.} and flexible distribution options.
%The model abstracts away many of the details of programming multiple address spaces while allowing users to fine-tune the distribution of work and data among devices in different nodes. 

The \name\ provides automatic communication when supplied with annotations providing work distribution and the data needed by the work. The annotations allow the specifications of the data read and written during kernel invocations. The specifications can also provide \emph{offset}s which refer to data boundary relative to each OpenCL work item, and for a large class of kernel code, these offsets are easy for programmers to provide.  As well, \name\ supports explicit and implicit partitioning of work item regions across devices. With offset and partition information, the \name\ runtime automatically generates efficient communication. This relieves programmers from handling explicit communication, allowing them to focus on kernel programming. Furthermore, \name~allows programmers to distribute data and work separately through APIs using a partitioned work item region ID. Therefore, there is no data ownership, and programmers can selectively use different partitions for both data and work at any program point. This flexibility allows programmers to optimize work distribution, and therefore communication, without any modification of existing kernel code. 
\fi

To summarize, our contributions are 
\begin{enumerate}
	\item A novel and easy programming model that can efficiently run on distributed heterogeneous devices, enabling flexible work distribution, with data flowing to the work that needs it.
	\item A fully automatic runtime communication generation scheme and its implementation.
	\item A flexible user interface that allows manual tuning of work distribution for high performance and enabling automatic communication. 
	%The interface lets users utilize device resources to balance workloads and manually distribute data to reduce communication cost.
	% \item A runtime system that is maintainable and extensible. We also discuss the overheads of the runtime system and opportunities for improvement.
	\item Experimental results showing good performance and speedups on small clusters with eight nodes and 1 to 32 GPUs.
\end{enumerate}

The rest of the paper is organized as follows. 
Sections~\ref{s:design}, ~\ref{subs:ui}, and~\ref{s:impl} describe the design and implementation of the \name~interface. Section~\ref{s:eval} presents a performance evaluation of the \name~runtime system. Section~\ref{s:related} discusses related work, and conclusions and future work follow in Section~\ref{s:conclusion}. 



==> arxiv_hdarray/related.tex <==
Our paper is related to previous efforts to simplify distributed accelerator programming with runtime support for efficient communication.
%
%\subsection{Programming Models for Accelerator Clusters}
\label{subs:related_acc_cluster}
%Although OpenCL and MPI are portable, the low-level APIs force users to explicitly manage communication and data distribution. 
%
Hydra~\cite{sakdhnagool2015hydra} is a compiler-assisted runtime system which extends OMPD~\cite{Kwon:2012:HAO:2145816.2145827}'s hybrid compiler-runtime communication analysis to  translate and execute OpenMP programs on accelerator clusters. One difference is that \name\ handles communication without any static analysis, allowing programmers to use separate compilation and external binary libraries.% as long as they update arrays through \funcread\ and \funcwrite\ calls.

%UPC~\cite{upc2005upc}, Co-array Fortran~\cite{numrich1998co}, and X10~\cite{charles2005x10} are Partitioned Global Address Space (PGAS) languages that expose a global shared array 
% so that a programmer can partition the array without worrying about the communication. 
PGAS languages~\cite{upc2005upc, numrich1998co, charles2005x10}
%These 
%programming paradigms 
have been extended to support accelerator clusters~\cite{Lee:2011:EXP:2238356.2238410, potluri2013extending, 7081675}.
PGAS languages expose a global shared array to relieve programmers from data distribution and communication handling but require the  specification of the affinity between data and threads, which makes data owned by a thread. As the data ownership is strongly coupled with computation, changing data distribution may require the modification of computation code. Our approach gives more freedom to the programmer to re-distribute data at any parallel program point without changes in kernel code. High Performance Fortran (HPF)~\cite{RiceUniversity:1993:HPF:174223.158909, Gupta:1995:HCI:224170.224422}
% also provides a global address space programming model that runs on clusters~\cite{RiceUniversity:1993:HPF:174223.158909, Gupta:1995:HCI:224170.224422}. Programmers explicitly distribute data using HPF directives, which guides computation partitioning and communication handling. HPF 
does not support accelerators.

Researchers have proposed language extensions for the programmability of heterogeneous clusters. SnuCL~\cite{kim2012snucl} and SnuCL-D~\cite{kim2016distributed} enable OpenCL applications to run in a distributed manner without any modification. 
% by making all the devices on a cluster logically appear on a single local node. 
dCUDA~\cite{gysi2016dcuda} automatically overlaps on-node computation and inter-node communication with hardware support and device-side remote memory access operations. It combines the MPI and CUDA programming models into a single CUDA kernel. IMPACC~\cite{kim2016impacc} integrates MPI and OpenACC~\cite{openacc} while exploiting shared memory parallelism. It reduces the communication cost through unified MPI communication routines, a unified node virtual address space, node heap aliasing technique, etc. Despite their optimized communication with little or no code changes, programmers are forced to manage numerous low-level details of the accelerator or MPI programming because these tools provide an abstraction level analogous to OpenCL/CUDA or MPI, and require explicit data transfer or communication code.

OmpSs~\cite{bueno2012productive} supports task parallelism and directives for computation offloading and communication handling. Programmers specify accessed regions of shared data, but no convenient way to define and operate on subarrays is provided. We differ by supporting data parallelism and allowing users to specify per-thread offset information, 
% which can be easily derived for regular applications, 
and both work and data partitioning can be done automatically or manually.
%
HOMP~\cite{yan2017homp} proposes an extension of OpenMP for distributing and binding computation and data, which gives users more control of managing data and computation, but 
% It also provides a number of loop distribution algorithms for better load-balancing. Unlike~\name, HOMP 
lacks cluster support and manual partitioning for specific devices.

Vi{\~n}as \textit{et al}.~\cite{vinas2016towards} proposed the hybrid use of Hierarchically Tiled Array (HTA)~\cite{bikshandi2006programming} for globally distributed arrays and Heterogeneous Programming Library (HPL)~\cite{vinas2013exploiting} for accelerators. Both HTA and HPL C++ libraries provide implicit parallelism and communication and hide many low-level details of MPI and OpenCL; however, there exist two different arrays: an HTA and an HPL Array, which programmers need to define and maintain. Explicit data transfer from the HPL Array to an HTA is also necessary.
%
PARRAY~\cite{Chen:2012:PUA:2145816.2145838, cui2015programming} is a C language extension that introduces novel array types to separate the logical and physical structure and what kind of process/thread will operate on a dimension. 
% using a very flexible notation with a Single-Program-Multiple-Codeblock (SPMC) programming style. The data array type separates the physical storage and logical structure of data to support logical multi-dimensional array operations. The thread array type indicates what kind of process/thread will be used for the array dimensions to unify various communication mechanisms (MPI, Pthread, CUDA, or other optimized libraries, e.g., PGAS calls). 
Unlike \name, users need to specify communication mechanisms for every array and explicitly insert communication code. 

Skeleton libraries~\cite{ernsting2017data, majeed2013cluster} % are another approach to exploit accelerator clusters with less programming effort. One limitation is that 
differ from us in that they can only support applications in which all the computational patterns are covered by the skeletons.
%
%\subsection{Easier Accelerator Programming}
Other popular platforms such as
%Accelerators offer highly-efficient parallelism which makes it an attractive target for computing intensive applications. 
% Due to the difficulty of programming accelerators, systems to make this easier have been proposed.
%for leveraging their computational resources. 
% One approach is enabling accelerator programming in simple scripting languages. 
NumbaPro~\cite{numbapro}, Arrayfire~\cite{arrayfire}, PyCUDA~\cite{KLOCKNER2012157},  Copperhead~\cite{Catanzaro:2011:CCE:1941553.1941562},  
% support Python libraries for accelerators. 
OpenACC
and 
% is an OpenMP-like directive-based accelerator programming model. 
OpenMP 4.0 % 
all aim to make accelerator programming easier, but only target a single node.
% includes the OpenACC feature. Unlike \name, all of these APIs and programming models target  a single node.

%The availability of accelerators and large data sets make Machine Learning increasingly popular. 
%%To meet the high demand for an easy 
%To facilitate programming environment for Machine Learning applications, many frameworks are already available. Most of them are Python-based Deep Learning frameworks~\cite{chintala2017overview, jia2014caffe, tokui2015chainer, 45166}. 
%%TensorFlow~\cite{45166} uses graph-based task parallelism and also supports distributed systems but is not publicly available. 
%%\Mycomment{What is not publically available?  The reference contains a download link.} \Hyundokcomment{I meant that the distributed version of Tensorflow was not free software, but I am replacing the sentence with the following:}
%Those applications are mostly array-centric and fit our purpose of parallelizing array-based programs. Our future work will be based on our experience of running and evaluating a deep learning neural network on the \name\ interface.

%\subsection{Efficient communication with runtime support}
%\begin{enumerate}
%	\item better communication performance
%	\begin{enumerate}
%		\item NVIDIA Collective Communications Library (NCCL2)~\cite{nccl}
%		\begin{enumerate}
%			\item better collective communications. Exploits NVLINK and gpu topology.
%			\item Users still need to specify the communication pattern like MPI programming
%		\end{enumerate}
%	\end{enumerate}
%\end{enumerate}

%\subsection{Contrast in emphasizing}
%\begin{enumerate}
%	\item Multi-node support.
%	\item Easy data partitioning programming. Data partitioning code is independent of  computation code by composing DEF/USE.
%	\item Easy and efficient communication with the runtime support.
%	\item Various accelerator supports like OpenCL kernel programming.
%\end{enumerate}

%\subsection{Partitioned Global Address Space (PGAS)}
%\begin{enumerate}
%	\item Berkeley Unified Parallel C (UPC)
%		\begin{enumerate}
%			\item Referencing a remote shared memory translates into a communication.
%			\item No accelerator work.
%			\item  No update since 2012. (from their official website.)
%		\end{enumerate}
%	\item Coarray Fortran, X10, Titanium
%	\item References are available in the OMPD paper
%\end{enumerate}

%\subsection{High performance fortran}
%\begin{enumerate}
%	\item Old, but most extensive research was done.
%	\item Data distribution over a loop.
%	\item a process owns a partitioned data.
%		\begin{enumerate}
%			\item In our approach, no hard-wired ownership.
%		\end{enumerate}
%	\item Our approach is different in that we try separating the per-element computation from the data distribution. This gives application writers a big freedom to experiment data partitioning with ease.
%	\item No active work to support accelerators.
%	\item References are available in the OMPD paper.
%\end{enumerate}

%\textbf{\subsection{Accelerator programming}
%\begin{enumerate}
%	\item OpenCL
%	\item CUDA
%	\item It is very difficult to write a program with multi nodes.
%\end{enumerate}}

%\textbf{\subsection{For better accelerator programming (faster or easier)}
%\begin{enumerate}
%	\item Python for accelerator
%	\begin{enumerate}
%		\item numbapro~\cite{numbapro}
%		\item Arrayfire~\cite{arrayfire}
%		\item pyCUDA~\cite{pycuda}
%		\item copperhead~\cite{copperhead}
%	\end{enumerate}
%	\item OpenACC~\cite{openacc}
%		\begin{enumerate}
%		\item for single node.
%		\item similar to OpenMP. 
%		\item OpenMP 4.0 includes openacc features. 
%		\end{enumerate}
%	\item Pythan for Machine Learning
%		\begin{enumerate}
%		\item python is getting more popular.
%		\item More array centric programming.
%		\item frameworks
%			\begin{enumerate}
%				\item TensorFlow, Pytorch, Caffe, RIP, Chainer, CNTK, DSSTNE, DyNet, Keras, Mxnet, ...
%			\end{enumerate}
%		\item Mostly, single node work. TensorFlow has a support for multinodes, but not open, available only for paid users. Multinode supports are usually done on the graph node level.
%		\end{enumerate}
%	\item better communication performance
%		\begin{enumerate}
%			\item NVIDIA Collective Communications Library (NCCL2)~\cite{nccl}
%				\begin{enumerate}
%					\item better collective communications. Exploits NVLINK and gpu topology.
%					\item Users still need to specify the communication pattern like MPI programming
%				\end{enumerate}
%		\end{enumerate}
%\end{enumerate}}

